Shape-Space Deformer: Unified Visuo-Tactile Representations for Robotic Manipulation of Deformable Objects

Accurate modelling of object deformations is crucial for a wide range of robotic manipulation tasks, where interacting with soft or deformable objects is essential. Current methods struggle to generalise to unseen forces or adapt to new objects, limiting their utility in real-world applications. We propose Shape-Space Deformer, a unified representation for encoding a diverse range of object deformations using template augmentation to achieve robust, fine-grained reconstructions that are resilient to outliers and unwanted artefacts. Our method improves generalization to unseen forces and can rapidly adapt to novel objects, significantly outperforming existing approaches. We perform extensive experiments to test a range of force generalisation settings and evaluate our method's ability to reconstruct unseen deformations, demonstrating significant improvements in reconstruction accuracy and robustness. Our approach is suitable for real-time performance, making it ready for downstream manipulation applications.

==> chapters/03-problem_formulation.tex <==
% \section{Problem Formulation \& Dataset} 
% \cred{this section needs to go. }
    % \hl{Is this section required? Kind of} \\
    % Give a one sentence motivating the goal
    % Robotic manipulation of material in natural environments such as tree branches requires neogiating deformable objects, whether it is the task in question, such as a gardening task where trees must be plied and cut, and/or to displace obstacles, such as a fruit-picking task where branches and leaves obstruct a robot end-effector (EE) from reaching a target fruit. Our goal is to develop an efficient and generalisable method for modeling object deformation from EE interation, to predict the effect of robotic manipulation actions. \\
    % Our problem formulation is similar to \cite{Youngsun_2022_VIRDO}, however with tougher constraints to advance towards a real-time application environment.
    % The dataset consists of $\numObjs$ objects $\mathcal{O}_{i}$, with a nominal (undeformed) point cloud $\PcdSym_{i, \text{nom.}}$, and $\numDefs$ unique samples of deformed point clouds $\PcdSym_{i, j}$, resulting from a force $\ForceSym_{j}$ applied to the nominal shape at contact points $\ContactSym_{j}$.
    % %
    % $$\text{Dataset } = \{\mathcal{O}_{1},\; ..., \mathcal{O}_{\numObjs}\}$$
    % %
    % Where:
    % % $$ \mathcal{O}_{i} = \{ \PcdSym_{i, \text{nom.}}, \; (\PcdSym_{i, 1}, \ForceSym_{i, 1}, \ContactSym_{i, 1}), \, ..., \, (\PcdSym_{i, \numDefs}, \ForceSym_{i, \numDefs}, \ContactSym_{i, \numDefs}) \} $$
    % % or perhaps:
    % \begin{align*}
    %     \mathcal{O}_{i} &= \{
    %         \mathcal{D}_{i, \text{nom}}, \; 
    %         \mathcal{D}_{i, 1}, \; 
    %         ..., \;
    %         \mathcal{D}_{i, \numDefs}
    %     \} \text{ is an object.} \\
    %     \mathcal{D}_{ij} &= (\PcdSym_{ij},\; \ForceSym_{ij},\; \ContactSym_{ij}) \text{ is a single deformation.}
    % \end{align*}
    % \\
    % In the environment, a robot agent approaches an object to manipulate, and captures a nominal (undeformed) point cloud of the object surface $\mathbf{P}$ using a LIDAR/depth sensor. We assume that the point cloud gives an unobstructed view with high enough sampling to generate a watertight mesh of the object. A watertight mesh is necessary for determining what points in 3D space are inside or outside of the object. With this, a signed distance field SDF$(\mathbf{q})$ can be computed for query points $\mathbf{q}$ in the sample space $\bf{\Omega} \subset \mathbb{R}^3$. It should be understood that points on the object surface $\mathbf{p} \in \mathbf{P}$ form a zero level-set defined by SDF$(\mathbf{p}) = 0$. \\
    % In the environment, a robot agent approaches an object to manipulate, and captures a nominal (undeformed) point cloud of the object surface $\PcdSym$ using a LIDAR/depth sensor.
    % \hl{This section needs quite a bit of changing.} \\
    % We assume that the point cloud gives an unobstructed view with high enough sampling resolution to generate a watertight mesh of the object. We also assume that the force applied and contact locations from the robot EEF can be accurately obtained from a force torque sensor. \\
    % A watertight mesh is necessary for determining what points in 3D space are inside or outside of the object.
    % With this, a signed distance field SDF$(\QuerySet)$ can be computed for a set of query points $\QuerySet$ in the sample space $\SampleSpace \subset \mathbb{R}^3$. The points on the object surface $\mathbf{p} \in \PcdSym$ form a zero level-set defined by SDF$(\mathbf{p}) = 0$. \\
    % The objective of the model is to predict how the points in $\PcdSym_{i, \text{nom}}$ will be displaced into a deformed point cloud $\PcdSym_{i, j}$, given a force vector $\ForceSym_{i, j}$ applied by the robot EEF to contact locations $\ContactSym_{i, j} \subset \PcdSym_{i, j}$.
    % The same conditions of $\PcdSym$ being unobstructed, watertight and thus SDF-computable, are assumed for $\mathbf{D}$. 
    % In training, for each shape we choose a subset of 
    % We seek a method that can efficiently represent both the nominal shapes $\mathbf{P}_{i}$ as well as deformed shapes $\mathbf{D}_{i, j}$. Consider a dataset of $n$ unique 3D objects $\mathbf{O}_{1}, ..., \mathbf{O}_{n}$. Each object $i$ has a nominal shape $\mathbf{P}_{i}$, as well as $m$ deformed shapes $\mathbf{D}_{i, 1}, ..., \mathbf{D}_{i, m}$. Each deformation $j$ of an object $i$ has an associated force applied $\vec{u}_{i, j}$ and contacts $\mathbf{Q}_{i, j}$, which transforms the nominal shape $\mathbf{P}_{i}$ into the deformed shape $\mathbf{D}_{i, j}$. In VIRDO the problem formation is the same as described so far, with a training dataset containing all deformations \cite{Youngsun_2022_VIRDO}. With our method what we seek to extend, is the ability to generalise to unseen forces and contact locations. Our method will be deemed a success if trained on a dataset with some of the deformation instances withheld, and then able make accurate predictions from the withheld forces.
    % We seek a method that can efficiently represent both nominal and deformed shapes from a dataset of $n$ unique 3D objects. Each object $i$ has a nominal point cloud $\PcdSym_{i}$, as well as $m$ deformed point clouds $\mathbf{D}_{i, 1}, ..., \mathbf{D}_{i, m}$. Each deformation $j$ of an object $i$ has an associated force $\ForceSym_{i, j}$ applied and contacts  $\ContactSym_{i, j}$, which translates the points of $\PcdSym_{i}$ into $\mathbf{D}_{i, j}$. 
    % Previous work, for example~\cite{Youngsun_2022_VIRDO}, applied a similar problem formation as described, our primary difference is a training dataset containing all deformations, rather than only the nominal shape representation. With our method we seek the ability to generalise to unseen forces and contact locations. 
    % Previous work, for example~\cite{Youngsun_2022_VIRDO}, applied a similar problem formation as described, our primary difference is instead of the training dataset containing all deformations evaluated in testing, we seek the ability to generalise to unseen forces and contact locations, withholding some deformation instances in training.
    %Our method will be deemed a success if trained on a dataset with some of the deformation instances withheld, and then able make accurate predictions from the withheld forces.


==> chapters/031-background.tex <==
\section{Background}
    % \subsection{Neural Fields}\label{sec:Neural_Fields}
        % Cut this paragraph/section possibly: \\
        % Neural fields show promise with foundation models in replacing hand-engineered steps, which have the drawback of typically involving discrete or discontinuous transforms of data (e.g KNN clustering of point clouds for features) preventing gradients from propagating when training neural network components. An earlier alternative which permits full propagation of gradients is an end-to-end approach. If helpful to the overall task, there would ostensibly be similar kinds of transformations performed somewhere in the layers of the network, and possibly in a more optimal manner. What is lost however, is interpretability. Where exactly these analogues to hand-engineered steps are taking place in the end-to-end network is very difficult to ascertain, due to the number of parameters in neural networks and how they are optimised. Supposing that a downstream neural network module can be trained to perform similarly to the hand-engineered step, this module would be preferable because it allows gradient propagation while having a defined purpose. FIND EXAMPLE \\    
        % What is useful about a neural field module, is that if it is capable of replacing a hand-engineered step, then it can be pretrained to perform this step,  and then have its parameters frozen and used as a component module in the ML pipeline. Owing to the continuity of neural networks, gradients can naturally pass through the neural field when training other modules in the pipeline, while at the same time no interpretability of the pipeline has been lost. This strength of neural fields is taken advantage of in the related work, especially \cite{Youngsun_2022_VIRDO}.
        % $\hdots$
    \subsection{Implicit Neural Fields for Shape Representation}\label{subsec:Shape_Rep}
        % Neural fields for modelling 3D geometry have found success in circumventing the limitations faced by point clouds, meshes and voxels, of being discrete, non-canonical, and sparse. Particularly, the Signed Distance Field/Function (SDF) presents a convenient shape representation approach to be modelled by neural fields. For an object with volume $V$ and surface $\partial{}V$, its SDF (which we will define SDF$_{V}$), gives the distance between an input query point $\mathbf{q}$ and the closest point on the object surface $\mathbf{p} \in \partial V$, however with a negative sign if $\mathbf{q}$ is within the object volume, and positive sign if outside. By definition, any point on the object surface will return an SDF value of zero, allowing the object surface to be described implicitly as the zero level set $\partial V = \{ \mathbf{p} \in \mathbb{R}^{3} \; : \; \text{SDF}(\mathbf{p}) = 0 \}$.
        Neural fields for modelling 3D geometry have successfully addressed the drawbacks of point clouds, meshes and voxels, which are discrete, non-canonical, and sparse. The Signed Distance Field/Function (SDF) is particularly effective as a shape representation method using neural fields. It defines the distance from any point $\mathbf{x}$ to the nearest surface point $\mathbf{p}$ on the boundary $\partial{}V$ of an object  with volume $V$. This distance is negative if $\mathbf{x}$ is inside the object and positive if outside, which is why it is termed "signed". At the surface of the object, the SDF is zero, meaning the object's surface is implicitly described by the zero level set $\partial V = \{ \mathbf{p} \in \mathbb{R}^{3} \; : \; \text{SDF}(\mathbf{p}) = 0 \}$. 
        
        \cred{Is the equ in this parag useful for our method, are we using the notations?}
        
        % \begin{align} \tag{1}
        %     \text{SDF}:\mathbb{R}^{3}\rightarrow\mathbb{R}, \quad \text{SDF}(\mathbf{q})&:=\left\{\begin{array}{lr}
        %         -||\mathbf{q} - \mathbf{p}||, \; \text{if } \mathbf{q} \in V \\
        %         +||\mathbf{q} - \mathbf{p}||, \; \text{if } \mathbf{q} \notin V
        %     \end{array} %\right\}
        % \end{align}
        %
        % Being continuous neural networks, SDF neural fields have the freedom to be queried at any point in $\mathbb{R}^3$, with arbitrary precision, interpolating-within and exterpolating-outside points seen in the training data-set. Along with describing the surface, SDFs give useful information about how far away from the surface a given point is, which has found applicability in robotics tasks such as rigid manipulation \cite{Liu_2022_ReDSDF} and trajectory planning \cite{Camps_2022_Learning, Ortiz_2023_iSDF2022}. Furthermore, SDFs have the property of being continuous and differentiable over the input space $\hdots$
        % DeepSDF \cite{Park_2019_CVPR} made a pioneering contribution to 3D shape representation literature, introducing the concept of learning continuous Signed Distance Field/Functions (SDFs) with neural networks.

    \subsection{Latent Shape Representations } % \label{subsec:}
        As mentioned in Section~\ref{subsec:Shape_Rep}, an SDF neural field that takes an input point $\mathbf{x}$ and outputs $s$ is limited to representing the surface of a single shape. To allow a neural field to depict multiple shapes and effectively leverage common features during training, a latent parameterization of the shapes is typically used, as demonstrated in several studies~\cite{Park_2019_CVPR, Deng_2021_CVPR, Youngsun_2022_VIRDO}. Specifically, in addition to the input query point $\mathbf{x}$, a latent code $\alpha \in \mathbb{R}^{\latentSize}$ which is associated with a specific shape in the dataset, conditions the model. This model is expressed as $\text{SDF}_{\alpha}(\mathbf{x})$. These latent codes, $\alpha_{i}$, are parameters optimized during training that the SDF model must 'decode' to accurately represent a specific shape, known as an auto-\emph{decoder} architecture~\cite{Park_2019_CVPR}. \\
        \hl{Very stuck on what else to say here.}

    \subsection{Implicit vs. Explicit Use of Neural Fields}
        \hl{This section may have to go} \\
        A neural field is classified as explicitly used when the learned function outputs the desired result for a specific application without requiring an extraction process. For instance, consider learning the Signed Distance Function (SDF) of a scene, which can have implicit or explicit uses. If the objective of learning the SDF is to determine if waypoint locations are unoccupied (indicated by $\text{SDF}(\mathbf{x}) > 0$) for a robotic agent to navigate, then the SDF is utilised \emph{explicitly}. On the other hand, if the goal is to reconstruct the scene's surface geometry by extracting surface points $\mathbf{x}_{1}, \mathbf{x}_{2}, \dots$ satisfying $\text{SDF}(\mathbf{x}) = 0$, this usage is considered \emph{implicit}. \\
        \\
        In an explicit setup, the output is used directly, simply evaluating the condition $\text{SDF}(\mathbf{x}) > 0$, which ensures that each input value $\mathbf{x}$, receives a boolean true/false as its output. In contrast, the implicit approach offers no \emph{guarantees} regarding how many input values (if any) meets the condition $\text{SDF}(\mathbf{x}) = 0$, nor about the location of these points and the extent of sampling needed to identify or approximate them. This distinction becomes particularly relevant when considering the use of deep learning architectures in neural fields, noted for their low interpretability (\hl{what should I cite here?}). \\
        \\
        Floating artifacts clearly demonstrate the aformentioned limitation of using implicit neural fields \cite{seita2021learning, } regarding lack of guarantees. However, this issue has been mitigated in surface reconstruction tasks due to the availability of sufficient training samples and advancements that allow for much more extensive sampling \cite{ }. \\
        \\
        \hl{Could also mention that implicit use case leave a discontinuity in the differentiation chain at the extraction step $\rightarrow$ must optimize before on the function values and must have samples of this function's (input, output). } \\
        % Alternative:
        % Take the example of learning an image's colour function $\text{Img}(x, y)=(r, g, b)$. If the motive for learning this function is to have a compact representation for later reconstructing the image by querying a grid of pixels, then this is \emph{explicit}. Conversely, if the purpose is to discover locations in an image that are a certain colour $\mathbf{c}$, achieved by grid sampling to find points $(x_i, y_i)$ satisfying $\text{Img}(p_x, p_y)=\mathbf{c}$, then this is \emph{implicit}. \\
        \\
        
        % \input{tables/explicit_vs_implicit_fields}


    \subsection{Neural Fields for Shape Deformation} \label{subsec:Shape_Def}
        % DIF-Net $\hdots$ \\
        Deformation fields map the transformation between an undeformed shape $\mathbf{P}$ and its deformed state $\mathbf{P}'$. Commonly, this deformation is the result of a force field
        
        The deformation field function $\deformField{}:\mathbb{R}^{3}\rightarrow{}\mathbb{R}^{3}$ gives the deformation vector for a point $\mathbf{x}$ on $\mathbf{P}$ to move to its new location $\mathbf{x}' = \mathbf{x} + \deformField{}(\mathbf{x})$ on $\mathbf{P}'$. \\
        % \cite{Youngsun_2022_VIRDO}'s deform module, a neural field, takes an encoding of force and contact input to  \\
        \\
        Methods such as \cite{Youngsun_2022_VIRDO} use neural fields to model the deformation of objects for robotic manipulation. First, an object module similar to \cite{Park_2019_CVPR} models the Signed Distance Field (SDF) of nominal (undeformed) instances of an object. Then, a deformation module  models a vector field to displace points on the nominal object surface into the deformed instance. \\
        \\
        Explicit Neural Surfaces (ENS) presents a novel approach for 3D surface reconstruction, representing shapes as a mapping, deforming a unit sphere mesh into the shape \cite{walker2023ENS}. 
        \hl{}
        

==> chapters/backupmethod.tex <==
%saved on 15 sep 3 pm
\section{Methodology}
    %
    % Merge Observation and Unified Latent Representation boxes
    \begin{figure*}[t!]
        \centering
        \includegraphics[width=\textwidth]{figures/fig2_idea2.png}
        \caption{Given a known object class, contact locations and applied force, our method determines the corresponding deformation field. We create a unified representation of several objects and their deformation states, and a generate a surface reconstruction by explicitly learning the neural field from a template shape. }
        \label{fig:arch}
    \end{figure*}
    %
    In this section, we begin by elaborating on the architecture of our main network,  \cred{lets call our Network SSD stands for Shape-Space Deformer} $\mathcal{OD}$, which is designed to accurately represent the geometric variations across all observed $n \times m$ deformations.
    Each object is parameterized by embeddings $\alpha$, and the corresponding deformations are encoded by force codes $\mathbf{z}$.
    Fig.~\ref{fig:arch} depicts the proposed pipeline: starting from a known object class, contact locations and applied force, a shared shape representation is learned that encompasses all objects and their deformations, which are reconstructed by transforming a template shape.
    The initial sections explain the roles of these embeddings and force codes, setting the stage for explaining how these condition the behavior of $\mathcal{OD}$ to modelling each specific shape instance.
    This is followed by a detailed description of how these embeddings are initialized and optimized during training to capture the intrinsic geometric properties and deformation behaviors of the objects.
    %
\subsection{Unified Latent Representation} \label{subsec:latent}
    % \cred{
    % We focus this section on details of how we encode force and concatenate with object codes. \\
    % How object code gets defined in the first place (initialised from a given distribution use math if you can) \\
    % How we learn the template as opposed to set a template} \\
    % \\
    Our main network $\mathcal{OD}$ is used to represent the geometry of all $n\times{}m$ deformations contained within the dataset.
    To condition $\mathcal{OD}$ according to a particular object and deformation, we parameterise the $n$ objects with embeddings $\alpha$, and encode the $m$ deformations for each object with force codes $\mathbf{z}$.
    We first describe $\alpha$ and $\mathbf{z}$ before explaining the finer details of the conditioning.
    \\
    \\
    We represent the $i$'th object with $\alpha_{i}$, an embedding of length $l$, with $\alpha_{i}$ representing 'Object $i$' broadly, over both its nominal and deformed instances.
    The weights of each embedding are randomly initialised from a normal distribution $\sim\mathcal{N}(0.0,\, 0.1^{2})$, and then optimised throughout training with respect to the accuracy of $\mathcal{OD}$ (see~\ref{subsec:defLearning} and \ref{subsec:losses}).
    Thus, a latent space of objects is developed, positioning the embeddings $\alpha_{i}$ based on similarity of not only static geometric features, but also how the objects deform.
    \\
    \\
    For each deformation instance $j$ of an object, visuo-tactile input data is provided in the form of an applied force $\vec{u}_{j}$ and set of contact locations $\mathbf{C}_{j}$. Motivated by~\cite{Youngsun_2022_VIRDO}, we encode this input using a force encoder $F$ to produce a force code $\mathbf{z}_{j}$, expressed as:
    %
    \begin{align}
         F(\mathbf{C}_{j},\; \vec{u}_{j}) \;\; &= \;\; \mathbf{z}_{j} \; \in \; \mathbb{R}^{d} 
         \label{eq:forceCode} \\
         \nonumber{} \\
         % (\text{Object } i, \;\text{Deform } j) \;\; &\mapsto \;\; \alpha_{i}\oplus\mathbf{z}_{ij} \; \in \; \mathbb{R}^{l + d} \nonumber
         (\text{Object } i, \;\text{Deform } j) \;\; &\mapsto \;\; (\alpha_{i}, \;\mathbf{z}_{ij}) \; \in \; \mathbb{R}^{l + d} \nonumber
    \end{align}
    %
    The style of conditioning $\mathcal{OD}$ to represent multiple objects and deforms is referred to as a hyper-network, which is an MLP decoder, taking a latent conditioning vector as input and outputing either a set of weight layers to be transpanted into a main network \cite{NEURIPS2020_53c04118, Deng_2021_CVPR, Youngsun_2022_VIRDO}, or 'hyper-input' that is concatenated with outputs inside the layers of the main network (Fig.~\ref{fig:hypernet}).
    % The result is a network heavily characterised by the latent output.
    We concatenate $\alpha$ and $\mathbf{z}$ into a hyper-input for hyper-network $\Psi$, which decodes this into an output $\theta$ (Eq.~\ref{eq:hyperOutput}).
    The output $\theta$ is then joined with output from a hidden layer to condition the main network $\mathcal{OD}$ (Fig.~\ref{fig:hypernet}).
    We use the shorthand $\mathcal{OD}_{ij}$ to refer to the main network being conditioned on $\theta_{ij}$ from (object~$i$, deform~$j$).
    %
    \begin{align}
        % \theta_{ij} &= \Psi{}(\alpha_{i} \oplus \mathbf{z}_{j})
        \theta_{ij} &= \Psi{}(\alpha_{i},\; \mathbf{z}_{j})
        \label{eq:hyperOutput}
        % \mathcal{OD}_{ij}(\mathbf{x}) &\equiv \mathcal{OD}(\mathbf{x}, \theta_{ij})
    \end{align}
    %
    \begin{figure}[H]
        \centering
        \includegraphics[width=1\linewidth]{figures/hypernet.png}
        \caption{Our unified representation takes an object code and latent force vector to condition a single policy trained on all shape types and deformation examples to predict the augmentation to be applied to a cylindrical shape template.}
        \label{fig:hypernet}
    \end{figure}

\subsection{Deformation Learning}\label{subsec:defLearning}
    \cred{
    Deformation vector as opposed to scalar value $s$ in VIRDO \\
    Object code here too \\
    }
    %
    To represent geometry, our \OurMethod{} module $\mathcal{OD}$ learns a deformation field mapping query points in 3D space to an object's surface. similar to \cite{walker2023ENS}. 
    For an input point $\mathbf{x}$, $\mathcal{OD}$ returns a displacement vector $\vec{d}$, between $\mathbf{x}$ and the closest point $\mathbf{p}$ on the object surface $\mathbf{P}$ (Eq.~\ref{eq:OD_defn}). 
    Consequently, the surface point is simply this vector added to $\mathbf{x}$ (Eq.~\ref{eq:SurfPoint_formula}).
    For querying an entire set of points $\mathbf{X}$, we use the notation $\mathbf{X}' = \mathbf{X} + \mathcal{OD}(\mathbf{X})$.
    \begin{align}
        &\mathcal{OD} : \mathbb{R}^{3} \rightarrow \mathbb{R}^{3} \nonumber{} \\
        \nonumber{} \\
        \mathcal{OD}(\mathbf{x}) &= 
            \argmin_{ \mathbf{p} \in \mathbf{P} }{
                \big\{ \| \mathbf{p} - \mathbf{x} \| \big\}
            }
            \equiv \vec{d}
            \qquad \label{eq:OD_defn} \\
        \nonumber{} \\
        \mathbf{x}' &= \mathbf{x} + \mathcal{OD}(\mathbf{x}) \text{ yields surface points} \label{eq:SurfPoint_formula}
    \end{align}
%
\subsection{Getting to the Surface}
    \noindent{}Somewhat "free-form" writing here: \\
    \\
    %
    We present heuristics that motivate the application of $\mathcal{OD}$'s vector field both for representing surface geometry, and deformation from applied forces. 
    \\
    \\
    % Domain -> Codomain
    First, a salient observation is that the 'density' of points on an object surface is much less than the off-surface volume.
    By density, we mean in an applied sense, the number of sample coordinates in a dataset for neural field optimisation.
    Optimising $\mathcal{OD}$ is a \textbf{regression} problem, taking coordinates from the \emph{voluminous} domain of $\mathbb{R}^{3}$ and mapping them specifically onto an object \emph{surface}.
    The intent is that all outputs of $\mathcal{OD}$ relate explicitly to the surface.
    Contrast this with other neural fields (such as SDFs), which have no particular bias toward learning the surface.
    SDFs could be deemed a kind of \textbf{classifier}, assigning points from the same domain into three groups: the \emph{volume} outside of an object, the object surface, or inside the object \emph{volume}.
    \\
    \\
    A motivating property of the surface deformation field is its relationship with the surface normal field. On off-surface points, $\mathcal{OD}$ is equivalent to a scaled surface normal field.
    
    \cite{Yang_2023}
    % \begin{align}
        
    % \end{align}
    %
    %
    \subsection{Explicit NF Shape Rendering}\label{subsec:rendering}
        % \cred{in methodology section we better less refer to other methods instead explain the method proposed in this paper.} \\
        % Our \OurMethod{} module $\mathcal{OD}$ amalgamates the roles of the object ($\mathbf{O}$) and deformation modules ($\mathbf{D}$) from~\cite{Youngsun_2022_VIRDO}. Whereas an SDF is defined as the signed distance from the closest surface point, a \emph{scalar}, our \cred{do we say we are learning deformation field?}deformation field is defined as the displacement \emph{vector} $\vec{d}$ which transports $\mathbf{x}$ to the closest surface point.
        %
        The objective of mapping all of $\mathbb{R}^{3}$ to exclusively surface points is advantageous, because it removes the need to perform extraction algorithms on high-resolution grid samples to find (approximate) surface points.
        Instead, Equation \ref{eq:SurfPoint_formula} provides an \emph{explicit} formula to yield surface points.
        %
        \begin{figure}[t!]
            \centering
            \includegraphics[width=1\linewidth]{figures/cylinder_deform_triangles.png}
            \caption{Deforming a template mesh means that vertex connections are maintained.}
            \label{fig:triangles}
        \end{figure}
        %
        The object and force codes are given as a latent input, conditioning the network to represent different shapes and deformations.
        For the network to model (shape~$i$,~deformation~$j$) with latent input $(\alpha_{i}, \mathbf{z}_{j})$, we use the shorthand $\mathcal{OD}_{ij}(\mathbf{x})$.
        To render a mesh, we use $\mathcal{OD}$ to displace the vertices of a template cylinder mesh into the particular (shape, deformation) instance.
        A cylinder mesh is initialised to already have connected triangle faces (Fig.~\ref{fig:triangles}).
        %
    % \vspace{-2mm}
    % \subsection{Training} \label{subsec:training}
        % Both the neural network modules in our method ($\ODmod$ and $\ForceMod$), as well as the shape codes are trained end-to-end in a single stage. At each step, shape code $\ShapeCode$ is selected, the force module produces latent code $\ForceCode$, conditioning $\ODmod$ to estimate deformation vectors. A batch of $N$ query points $\QuerySet$ containing both on-surface and off-surface points are input to $\ODmod$, returning predicted deformation vectors values $\ODmod{}(\mathbb{Q}) = \widehat{\mathcal{Y}} \in \mathbb{R}^{N \times 1}$. Comparing ground truth SDF values with the output of the network, a loss $L$ was computed, and thus gradients to optimise the model parameters.
    %
\subsection{Losses} \label{subsec:losses}
    We employ geometric losses $L_{\text{vec.}}$ and $L_{\text{CD}}$ to learn accurate reconstructions of the nominal and deformed shapes, as well as regularisation losses for the latent codes $\ShapeCode$ and weights of $\ODmod$.
    %
    \begin{align}
        L = \lambda_{\text{vec.}} L_{\text{vec.}}
            +
            \lambda_{\text{CD}} L_{\text{CD}}
            +
            L_{\text{reg.}}
            % \lambda_{\alpha} L_{\alpha}
            % +
            % \lambda_{\mathbf{w}} L_{\mathbf{w}}
    \end{align}
    %
    \subsubsection{Geometry}
        %
        \begin{align}
            L_{\text{vec.}} &= \sum_{\mathbf{x} \in \Omega} 
            \big\|
                (\mathbf{x} + \mathcal{OD}(\mathbf{x})) - \mathbf{p}^{*}
            \big\|^{2}
            \\
            \nonumber{}
            \\
            L_{\text{CD}} &= \text{CD}(\mathbf{P}{\leftrightarrow}\mathbf{P}^{*})
            \label{eq:CDdef}
            \\
            \nonumber{}
            \\
            \text{Where:} \qquad \quad & \nonumber{}\\
            %
            \twoWayChamferSym{A}{B} &= \twoWayChamferDef{A}{B} \\
            \nonumber{}
            \\
            \oneWayChamferSym{A}{B} &= \oneWayChamferDef{A}{B} \quad \forall\mathbf{a}\in A
        \end{align}
    \subsubsection{Regularisation}
        We use two regularisation losses, one for regularising the latent shape codes ($L_{\alpha}$), and the loss $L_{\mathbf{w}}$ for regularisation of the weights of $\ODmod$. The two losses take the mean-squared sum of the shape codes and $\ODmod$ weights, encouraging the parameters to have a zero mean and low variance.
        \begin{align}
            &L_{\text{reg.}} = 
                \lambda_{\alpha}
                \text{ mean} \big( {\| \alpha \|}^{2} \big)
                + 
                \lambda_{\mathbf{w}}
                \text{ mean} \big( {\| \mathbf{w} \|}^{2} \big),
                \\
            &\forall \text{ shape codes } \alpha, \text{ and weights } \mathbf{w} \text{ from }  \mathcal{OD}. \nonumber{}
        \end{align}

==> chapters/figs/system_diagram.tex <==
\begin{figure}[!ht]
\centering
\resizebox{0.45\textwidth}{!}{

\begin{tikzpicture}
    \tikzstyle{every node}=[font=\LARGE]
    \draw  (10,11.25) rectangle  node {\LARGE $OD$} (15,8.75);
    \draw  (5,17.5) rectangle  node {\LARGE $F$} (7.5,12.5);
    \draw  (8.75,16.25) rectangle  node {\LARGE $z$} (10,13.75);
    \draw (7.5,15) to[short] (8.75,15);
    \draw  (12.5,15) circle (0.5cm);
    \draw [->, >=Stealth] (10,15) -- (12,15);
    \draw [->, >=Stealth] (12.5,14.5) -- (12.5,11.25);
    \draw  (8.75,21.25) rectangle  node {\LARGE $\alpha$} (10,18.75);
    \draw (10,20) to[short] (12.5,20);
    \draw [->, >=Stealth] (12.5,20) -- (12.5,15.5);
    \draw [short] (12.5,15.5) -- (12.5,14.5);
    \draw [short] (13,15) -- (12,15);

\end{tikzpicture}
}
\label{fig:my_label}
\end{figure}

==> chapters/tables/hero_image.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/rerank_fig1_dcc.png}
\caption{Example retrieval scenario where the top-1 retrieval (red) is not the same place as the query (blue) but the top-2 retrieval (green) is. Using re-ranking, the two retrievals can be re-arranged so that the query will match with the correct retrieval candidate. Examples from MulRan DCC dataset.}
\label{fig:hero_image}
\end{figure}

==> chapters/tables/main_pipeline.tex <==
\begin{figure*}[ht]
    \centering
    % \includegraphics[width=0.9\textwidth]{figures/new_pipeline2.png}
    \includegraphics[width=0.99\textwidth]{figures/reranking_black_revision.pdf}
    % \includesvg{figures/rerank.svg}
    \caption{\textcolor{blue}{Overview of our SpectralGV method}. Local features are extracted from the query point cloud using an encoder and then aggregated to form a global descriptor which is used in the `Retrieval' block to find the top-k place candidates (k=2 in the diagram). The local features and point cloud are used for  re-ranking the retrieved candidates in the `Re-Ranking' module which estimates a matching confidence based on the spatial consistency of point correspondences (black lines). 
    % Our re-ranking takes into consideration the local feature correspondences as well as how well their pairwise geometric constraints are satisfied. 
    In this example, retrieved point cloud `B' \textcolor{blue}{is more consistent with the query} and is therefore ranked higher than `A' after re-ranking.
    The 6DoF pose estimate \textcolor{blue}{$ \mathcal{T_B} $ is obtained by aligning the query point cloud to the top re-ranked candidate}. Point clouds are coloured based on the t-SNE embeddings of local features to better visualize the point correspondences. 
    % Best viewed in colour with zoom-in. better satisfies the geometric constrains
    }
    \label{fig:bl_pipeline}
\end{figure*}


==> chapters/tables/method_image.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/reranking-hero.pdf}
\caption{Visualization of values in the adjacency matrix $ M $. \textcolor{blue}{The colored lines represent inter-pointcloud correspondences. Out of the 3 depicted correspondences, the green ones ($c_1, c_3 $) are inliers and the red ($c_2 $) are outliers. The compatibility of these  correspondences are represented by the $m_{i,j}$ values in the top left of this figure.  Inlier correspondences will preserve their spatial consistency (low $d_{1,3}$) and form strong edges in $ \mathcal{G} $ (high $m_{1,3}$), while outliers will not form strong edges with the inliers (low $m_{1,2}$).}}
\label{fig:method_image}
\vspace{-5mm}
\end{figure}

==> chapters/tables/ntopk_plot.tex <==
% \begin{figure}[t]
% \centering
% %  trim={<left> <lower> <right> <upper>}
% % \includegraphics[width=0.499\textwidth, trim={3cm 2.5cm 2cm 3.5cm},clip]{figures/ntopk_plot_zoom.pdf}
% \includegraphics[width=0.48\textwidth, trim={0.5cm 2.5cm 0.1cm 3.0cm},clip]{figures/ntopk_plot3.pdf}
% % \includegraphics[width=0.48\textwidth, trim={0.5cm 2.0cm 0.1cm 3.5cm},clip]{figures/ntopk_plot2.pdf}
% \caption{\textcolor{blue}{Analysis of re-ranking methods with varying $ n_{topk} $ using the EgoNN architecture on the KITTI-360 dataset. SpecralGV shows consistently  increasing Recall@1 (green lines, left-side y-axis) while maintaining sub-linear time complexity (purple lines, right-side y-axis). }
% % $ n_{topk} = 1 $ is the baseline results without re-ranking.
% }
% % Analysis of re-ranking methods with varying $ n_{topk} $ using the EgoNN architecture on the KITTI-360 dataset. SpectralGV shows consistently increasing Recall@1 (green lines) with increasing $ n_{topk} $ while maintaining sub-linear time complexity (purple lines). 
% \label{fig:ntopk_plot}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%      \centering
%      \begin{subfigure}{\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/ntopk_methods_recall.pdf}
%          \caption{Recall@1 (\%)}
%          \label{fig:ntopk_plot_methods_recall}
%      \end{subfigure}
%      % \hfill
%      \begin{subfigure}{\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/ntopk_methods_time.pdf}
%          \caption{Re-Ranking Time (ms)}
%          \label{fig:ntopk_plot_methods_time}
%      \end{subfigure}
%         \caption{\textcolor{blue}{Analysis of re-ranking methods with varying $ n_{topk} $ using the EgoNN architecture on the KITTI-360 dataset. SpecralGV shows consistently  increasing Recall@1 (green lines, left-side y-axis) while maintaining sub-linear time complexity (purple lines, right-side y-axis). }}
%         \label{fig:ntopk_plot_methods}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\centering
%  trim={<left> <lower> <right> <upper>}
% \includegraphics[width=0.499\textwidth, trim={3cm 2.5cm 2cm 3.5cm},clip]{figures/ntopk_plot_zoom.pdf}
\includegraphics[width=0.99\linewidth]{figures/ntopk_methods_both_new2.pdf}
% \includegraphics[width=0.48\textwidth, trim={0.5cm 2.0cm 0.1cm 3.5cm},clip]{figures/ntopk_plot2.pdf}
\caption{\textcolor{blue}{Analysis of re-ranking methods with varying number of candidates used for re-ranking: $ n_{topk} $.
% using EgoNN on KITTI-360 09. 
SpectralGV shows consistently  increasing Recall@1 (left plot) while maintaining sub-linear time complexity (right plot).}}
\label{fig:ntopk_plot}
\vspace{-5mm}
\end{figure}

==> chapters/tables/qualitative_rerank.tex <==
\begin{figure*}[htb!]
     \centering
     \begin{subfigure}[b]{0.1949\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-label_sejong_qual_rr_dist.pdf}
         \caption{MulRan Sejong}
         \label{fig:qual_rr_sejong}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1549\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-apollo_qual_rr_dist.pdf}
         \caption{Apollo-Southbay}
         \label{fig:qual_rr_apollo}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1549\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-kitti_qual_rr_dist.pdf}
         \caption{KITTI 00}
         \label{fig:qual_rr_kitti00}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1549\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-dcc_qual_rr_dist.pdf}
         \caption{MulRan DCC}
         \label{fig:qual_rr_dcc}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1549\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-alita_qual_rr_dist.pdf}
         \caption{ALITA}
         \label{fig:qual_rr_alita}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.1549\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/reranking-360_qual_rr_dist.pdf}
         \caption{KITTI-360 09}
         \label{fig:qual_rr_kitti360}
     \end{subfigure}
    \caption{\textcolor{blue}{Visualizations of retrieval corrections by SpectralGV on the five datasets using the EgoNN architecture. Our re-ranking method is able to filter out incorrect initial candidates which are highly structurally similar to the query and correct them by accurately identifying the correct candidate. The distance of each retrieval to the query is noted in the text box.} 
    % \textcolor{red}{Top row shows the query, middle row shows the initial top1 retrieval (incorrect) and the bottom row shows the re-ranked top1 retrieval (correct). Point clouds are visualized from top-down orthogonal point of view and points are colored based on height.} 
    }
    \label{fig:quali_rerank}
\end{figure*}

==> chapters/tables/seq_eval.tex <==
\begin{table*}[htbp]
\begin{center}
\begin{tabular}{l@{\quad}|r@{\quad}r@{\quad}r@{\quad}r@{\quad}r@{\quad}r@{\quad}|r@{\quad}|r@{\quad}r@{\quad}r@{\quad}r@{\quad}r@{\quad}|r@{\quad}|r@{\quad}r|}
\cline{2-14}
&  \multicolumn{7}{c|}{KITTI} & \multicolumn{6}{c|}{MulRan} \\
\cline{2-14}
&  \begin{tabular}{@{}c@{}}00\end{tabular}
& \begin{tabular}{@{}c@{}}02\end{tabular}
& \begin{tabular}{@{}c@{}}05\end{tabular}
& \begin{tabular}{@{}c@{}}06\end{tabular}
& \begin{tabular}{@{}c@{}}07\end{tabular}
& \begin{tabular}{@{}c@{}}08\end{tabular}
& \begin{tabular}{@{}c@{}}mean\end{tabular}
& \begin{tabular}{@{}c@{}}K1\end{tabular}
& \begin{tabular}{@{}c@{}}K2\end{tabular}
& \begin{tabular}{@{}c@{}}K3\end{tabular}
& \begin{tabular}{@{}c@{}}D3\end{tabular}
& \begin{tabular}{@{}c@{}}R2\end{tabular}
& \begin{tabular}{@{}c@{}}mean\end{tabular}
\\[2pt]
\hline
% M2DP~\cite{He2016} & 0.836 & 0.781 & 0.772 & 0.896 & 0.861 & 0.169 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 \\
ScanContext~\cite{Kim2018} & 0.966 & 0.871 & 0.914 & 0.985 & 0.698 & 0.610 & 0.841 & 0.954 & \textbf{0.969} & \textbf{0.994} & 0.893  & 0.826 & 0.916 \\
% \hline
% \hline
PointNetVLAD~\cite{Uy2018} & 0.909 & 0.637 & 0.859 & 0.924 & 0.171 & 0.437 & 0.656 & 0.952 & 0.856 & 0.979 & 0.685 & 0.868 & 0.868 \\
Locus~\cite{vidanapathirana2020locus} & \textbf{0.983} & 0.762 & \textbf{0.981} & \textbf{0.992} & \textbf{1.000} & \textbf{0.931} & \textbf{0.942} & 0.938 & 0.874 & 0.969 & 0.718 & \textbf{0.994} & 0.899 \\ 
%MinkLoc~\cite{Kim2018}) & 00 & 00 & 00 & 00 & 00 &00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 \\
\textbf{LoGG3D-Net (Ours)}  & 0.953 & \textbf{0.888} & 0.976 & 0.977 & \textbf{1.000} & 0.843 & 0.939 & \textbf{0.966} & 0.938 & 0.991 & \textbf{0.977} & 0.969 & \textbf{0.968} \\
\hline
\end{tabular}
\end{center}
\caption{Evaluation of sequential place recognition on KITTI and MulRan datasets using $F1_{max}$ metric under the $3m,20m$ revisit criteria.
The rows are grouped as handcrafted, hybrid, and end-to-end learning-based respectively.}
\label{tab:seq_eval}
\end{table*}

%Locus~\cite{vidanapathirana2020locus} & \textbf{0.98} & 0.785 & \textbf{0.985} & \textbf{0.998} & \textbf{1.000} & \textbf{0.938} & \textbf{0.948} & 0.938 & 0.874 & 0.969 & 0.718 & \textbf{0.994} & 0.899 \\ 

==> chapters/tables/table_data_splits.tex <==
\begin{table}[t!]

\begin{center}
%@{\enspace}
\begin{tabular}{@{\enspace}l@{\enspace}|@{\enspace}r@{\enspace}|@{\enspace}c@{\enspace}|@{\enspace}c@{\enspace}}
%\hline
\begin{tabular}{@{}c@{}} Train/Test Split \end{tabular}
& \begin{tabular}{@{}c@{}}Length \end{tabular}
& \begin{tabular}{@{}c@{}}Step \end{tabular}
& \begin{tabular}{@{}c@{}}Number of scans\end{tabular}
\\[2pt]
\hline
% \Tstrut
\textit{Train split:}  &  &  \\
MulRan \cite{mulran20}: Sejong (0.1/02) & 19 km & 0.2 m & 35,871 \\
SouthBay \cite{apollo_dataset}: excl. Sunnyvale  &  37 km & 1.0 m & 72,706 \\
\hline
% \Tstrut
\textit{Test split (Easy):}  &  & & (database\,/\,query) \\
MulRan\cite{mulran20}: Sejong (01/02)  &  4 km & 0.2 m & 3,764\,/\,3,453 \\
SouthBay\cite{apollo_dataset}: Sunnyvale  &  38 km & 1.0 m & 48,959\,/\,16,999  \\
KITTI\cite{geiger2013kittidataset}: Sequence 00 & 4 km & 0.1 m & 1,620\,/\,621  \\
\textit{Test split (Hard):}  &  &  \\
MulRan\cite{mulran20}: DCC (01/02)  & 4.9 km & 10.0 m & 469\,/\,307  \\
ALITA\cite{yin2022alita} (val:5)  & 1.4 km & 3-20 m & 107\,/\,84  \\
KITTI-360\cite{liao2022kitti360}: Sequence 09  & 10.5 km & 3.0 m & 766\,/\,398  \\
\end{tabular}
\caption{Details of training and evaluation sets.}
\label{tab:data_splits}
\end{center}
\vspace{-6mm}
\end{table}
% \cred{Add heading title to col1 (Train/Test Split)}

==> chapters/tables/table_metloc.tex <==
\begin{table*}[hhtb!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}|c@{\quad}|c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
%\hline
&  \multicolumn{1}{c}{keypoint} &  \multicolumn{1}{c}{num} &  \multicolumn{1}{c}{feature} &  \multicolumn{4}{c}{MulRan Sejong} & \multicolumn{4}{c}{Apollo-SouthBay} & \multicolumn{4}{c}{KITTI} 
\\
& detection & points  & size
& \begin{tabular}{@{}c@{}}S \end{tabular}
& \begin{tabular}{@{}c@{}}RTE \end{tabular}
& \begin{tabular}{@{}c@{}}RRE \end{tabular}
& \begin{tabular}{@{}c@{}}t \end{tabular}
& \begin{tabular}{@{}c@{}}S \end{tabular}
& \begin{tabular}{@{}c@{}}RTE \end{tabular}
& \begin{tabular}{@{}c@{}}RRE \end{tabular}
& \begin{tabular}{@{}c@{}}t \end{tabular}
& \begin{tabular}{@{}c@{}}S  \end{tabular}
& \begin{tabular}{@{}c@{}}RTE \end{tabular}
& \begin{tabular}{@{}c@{}}RRE \end{tabular}
& \begin{tabular}{@{}c@{}}t \end{tabular}
\\[2pt]
\hline

% \Tstrut
% EgoNN+FCGF~\cite{choy2019fully} & 0.965 & \underline{18} & \textbf{0.4} & 0.943 & \underline{13} & \underline{0.4} & 0.966 & \underline{10} & \underline{0.3} \\
% EgoNN+D3Feat~\cite{bai2020d3feat} & \underline{0.991} & \textbf{16} & \textbf{0.4} & \textbf{0.975} & \textbf{12} & \textbf{0.3} & \textbf{0.998} & \textbf{7} & \textbf{0.2} \\
% Przeliczone dla DH3D dla threshold 1m 
DH3D*~\cite{du2020dh3d} & yes & 512 & 128 & 56.3 & 41 & 1.3 & - & 61.4 & 55 & 0.9 & - &  93.2 & 26 & 0.6 & - \\
% model: model_egonn_20210916_1104_final.pth
% Mulran: test_Sejong01_Sejong02.pickle
% SouthBay: Evaluation set: test_SunnyvaleBigloop_1.0_5.pickle
% kitti_00_eval.pickle
EgoNN~\cite{egonn} & yes & 128 & 128 & \underline{99.6} & \underline{19} & \underline{0.4} & \textbf{4} & 
\underline{99.9} & \textbf{15} & 0.4 & \textbf{1}  &
99.7 &  \underline{12} & \textbf{0.3} & \textbf{5} \\
% LCD-Net \cite{cattaneo2022lcdnet} \textbf{not trained} & yes & 4096 & 640 & 
% 0.825 & 29 & 0.7 & - & 
% 0.942 & 20 & 0.4 & 1,311 &
% 100 &  12 & 0.3 & 677 \\
LCDNet \cite{cattaneo2022lcdnet}  & yes & 4096 & 640 & 
87.2 & 26 & 0.6 & 682 & 
96.2 & 18 & \textbf{0.3} & 1,311 &
\textbf{100} &  \underline{12} & 0.4 & 677 \\
% \hline
LoGG3D-Net-sparse & no & $\sim N/8 $  & 81 & 
99.4 & 50 & 0.6 & \underline{12} & 
99.0 & 55 & 0.6 & \underline{20} &
99.8 &  34 & 0.5 & \underline{9} \\
LoGG3D-Net-dense & no & $ N $ & 32 & 
\textbf{99.8} &  \textbf{17} & \textbf{0.3} & 293 &
\textbf{100} & \textbf{15} & \textbf{0.3} & 159 &
\textbf{100} &  \textbf{10} & \textbf{0.3} & 99  \\

% [2pt]
\end{tabular}
\caption{Results of 6DoF pose estimation under the 2\,m and $5^\circ$ thresholds. `S'($\uparrow$) = Success rate (\%), `RTE'($\downarrow$) = Relative Translation Error (cm), `RRE'($\downarrow$) = Relative Rotation Error($^\circ$), `t'($\downarrow$) = pose estimation time (ms). `$N$' is the number of points input to the network after downsampling and ground-plane removal. (*) Results are obtained from \cite{egonn}. \textcolor{red}{try to do a hard eval to highlight keypoint-less advantage. replace this table with a met loc eval with and without reranking using all queries. }}
\label{tab:metric_loc}
\end{center}
\end{table*}

==> chapters/tables/table_metloc_rerank.tex <==
\begin{table}[htb!]

\begin{center}
%@{\enspace}
\begin{tabular}{@{\enspace}l@{\enspace}|@{\enspace}c@{\enspace}|@{\enspace}c@{\enspace}|@{\enspace}c@{\enspace}}
%\hline
\begin{tabular}{@{}c@{}}  \end{tabular}
& \begin{tabular}{@{}c@{}}S (\%) ($\uparrow$) \end{tabular}
% & \begin{tabular}{@{}c@{}} $\Delta$S  \end{tabular}
& \begin{tabular}{@{}c@{}}RTE (m) ($\downarrow$) \end{tabular}
& \begin{tabular}{@{}c@{}}RRE ($^\circ$) ($\downarrow$) \end{tabular}
\\[1pt]
\hline
% \Tstrut

EgoNN~\cite{egonn}  & 88.2 & 42.45 & 13.36 \\
LCDNet~\cite{cattaneo2022lcdnet} & 94.0   & 10.40 & 6.37  \\
LoGG3D-Net~\cite{vid2022logg3d} &  97.0  & 9.51 & 3.64 \\
\hline
EgoNN + SGV  & 98.7  & 4.32 & 1.44 \\
LCDNet + SGV  & 98.5   & \textbf{0.79} & 2.35 \\
LoGG3D-Net + SGV  &  \textbf{99.5}  & 2.88 & \textbf{1.07} \\

\end{tabular}
\caption{\textcolor{blue}{Results of 6DoF metric localization on the unseen KITTI-360 09 dataset with and without re-ranking}. 
% `S': Success rate (\%), 
% `$\Delta$S': increase in S after re-ranking, 
% `mRTE': mean Relative Translation Error (m), `mRRE': mean Relative Rotation Error($^\circ$).
}
\label{tab:met_loc_new}
\end{center}
\vspace{-6mm}
\end{table}

==> chapters/tables/table_placog.tex <==
\begin{table*}[ht!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
%\hline
&  \multicolumn{4}{c}{MulRan Sejong} & \multicolumn{4}{c}{Apollo-SouthBay} & \multicolumn{4}{c}{KITTI} & \multicolumn{4}{c}{Average}  \\
&  \multicolumn{2}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
&  \multicolumn{2}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
&  \multicolumn{2}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
&  \multicolumn{2}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
\\
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}R5\end{tabular}

\\[2pt]
\hline
MinkLoc3D*~\cite{Komorowski_2021_WACV} & 82.3 & 94.4 & 92.1 & 96.6 & 77.2 & 93.8 & 95.0 & 98.3 & 95.7 & 96.9 & 97.7 & 98.0 & 85.0 & 95.0 & 94.9 & 97.6 \\
DiSCO*~\cite{xu2021disco} & 94.0 & 97.5 & 95.8 & 98.1 & 
95.1 & 96.6 & 95.4 & 97.0 & 90.7 & 91.3 & 92.3 & 94.5  & 93.2 & 95.1 & 94.5 & 96.5 \\
DH3D*~\cite{du2020dh3d} & 32.4 & 56.2 & 58.9 & 75.5 & 25.3 & 49.6 & 50.4 & 70.7 &  75.5 & 91.1 & 86.8 & 96.1  & 44.4 & 65.6 & 65.3 & 80.7 \\
ScanContext~\cite{kim2018scan}  & 86.1 & 89.6 & 88.5 & 91.5 & 91.0 & 91.0 & 92.1 & 92.4 & 96.3 & 97.4 & 96.3 &  97.6  & 91.1 & 92.6 & 92.3 & 93.8 \\ 
Locus~\cite{vidanapathirana2020locus} & 	67.0 & 75.8 & 70.6 & 74.6 &  85.5 & 95.5 & 94.9 & 98.1 & 99.0 & 99.7 & 99.8 & \textbf{100}  & 83.8 & 90.3 & 88.4 & 90.9  \\
EgoNN~\cite{egonn} & 98.3 &  \textbf{99.9} &  \textbf{99.6} &  99.9 & 
95.7 & 97.7 & 96.3 & 98.2 & 
97.4 &  98.2 &  97.9 &  98.7
 & 97.1 & 98.6 & 97.9 & 98.9
 \\

LCDNet~\cite{cattaneo2022lcdnet} &  63.1 & 82.0 & 85.8 & 92.1 & 64.7 & 81.7 & 87.4 & 92.1  &  96.9 & 99.4 & 99.5 & 99.8  & 74.9 & 87.7 & 90.9 & 94.6  \\
LoGG3D-Net~\cite{vid2022logg3d} & 97.7 & 99.7 & 98.8 & 99.8 &  95.2 & 98.4 & 98.2 & \underline{99.2} &  \textbf{99.7} & \textbf{99.8} & \textbf{100} & \textbf{100}  & 97.5 & \underline{99.3} & 99.0 & \underline{99.6}  \\
\hline
EgoNN + SGV & \textbf{99.1} &  \textbf{99.9} &  \textbf{99.6} &  \textbf{100} & 
\underline{98.3} & \underline{98.7} & \underline{99.1} & \underline{99.2} & 
99.2 &  99.4 &  99.7 &  99.7  & \underline{98.8} & \underline{99.3} & \underline{99.4} & \underline{99.6}
 \\
LCDNet + SGV & 90.8 & 92.4 & 94.3 & 95.8 &  90.0 & 90.8 & 95.2 & 95.6 &  \textbf{99.7} & 99.7 & \textbf{100} & \textbf{100}   & 93.5 & 94.3 & 96.5 & 97.1 \\
LoGG3D-Net + SGV & \underline{99.0} & \textbf{99.9} & 99.5 & \textbf{100} &  \textbf{98.6} & \textbf{99.3} & \textbf{99.6} & \textbf{99.6} &  \textbf{99.7} & \textbf{99.8} & \textbf{100} & \textbf{100}  & \textbf{99.1} & \textbf{99.6} & \textbf{99.7} & \textbf{99.8} \\[2pt]
\end{tabular}
\caption{Place recognition on the `easy' evaluation set. 
% Recall@1 and Recall@5 are reported with 5 and 20\,m thresholds. 
(*) Results are obtained from \cite{egonn}. `R1': Recall@1, `R5': Recall@5.
% Bold and underline represent the best and 2nd best result respectively in each column.
}
\label{tab:place_recog_easy}
\end{center}
\end{table*}

==> chapters/tables/table_placog_hard.tex <==
\begin{table*}[ht!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
%\hline
&  \multicolumn{5}{c}{MulRan DCC} & \multicolumn{5}{c}{ALITA} & \multicolumn{5}{c}{KITTI-360}  \\
&  \multicolumn{3}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
&  \multicolumn{3}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 
&  \multicolumn{3}{c}{5\,m } & \multicolumn{2}{c}{20\,m } 

\\
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}} $\Delta$MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}$\Delta$MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}$\Delta$MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}


% Ew. dodać liczbę iteracji RANSACa jak w DH3D
\\[2pt]
\hline
ScanContext~\cite{kim2018scan}  & 	72.0 & 80.5 & - & 93.2 & 94.0  & 57.1 & 66.5 & - & 59.5 &  69.4  & 93.7 & 94.9 & - &  	95.2 & 	95.9   \\
Locus~\cite{vidanapathirana2020locus}  & 46.3 & 55.6 & - & 71.0 & 77.5  & 95.2 & 97.6 & - & \textbf{100} &  \textbf{100}  & 92.7 & 95.1 & - &  97.0 & 98.1   \\

EgoNN~\cite{egonn}  & 67.1 & 77.2 & - & 90.2 & 92.3  & 79.8 & 87.3 & - & 91.7 &  94.9  & 86.9 & 90.1 & - &  88.2 & 91.4   \\
LCDNet~\cite{cattaneo2022lcdnet} & 57.7 & 71.6 & - & 90.9 & 93.8 &  
90.5 & 94.6 & - & 96.4 & 97.8 &  
85.9 & 89.7 & - & 95.7 & 96.6   \\
LoGG3D-Net~\cite{vid2022logg3d} & 66.8 & 76.7 & - & 91.2 & 92.9 &  
15.5 & 28.0 & - & 26.2 & 40.0 &  
93.2 & 95.5 & - & 97.5 & 98.1   \\
\hline
 EgoNN + SGV & \underline{73.6} & \textbf{82.2} & 5.0 & 95.1 & 95.7  & \textbf{100} & \textbf{100} & 12.7 & \textbf{100} &  \textbf{100}  & \underline{95.7} & \underline{96.9} & 6.8 &  98.7 & 98.8   \\
LCDNet + SGV & 72.3 & 83.0 & 11.4 & \textbf{99.3} & \textbf{99.4} & 
\textbf{100} & \textbf{100} & 5.4 & \textbf{100} & \textbf{100} &  
\underline{95.7} & 96.2 & 6.5 & \underline{99.0} & \underline{99.1}   \\
LoGG3D-Net + SGV & \textbf{73.9} & \underline{82.0} & 5.3 & \underline{96.1} & \underline{96.5} &  
60.7 & 63.2 & 35.2 & 75.0 & 77.3 &  
\textbf{96.7} & \textbf{98.1} & 2.6 & \textbf{99.5} & \textbf{99.5} \\[2pt]
\end{tabular}
\caption{Place recognition on the unseen `hard' evaluation set. 
% Recall@1 and MRR are reported with 5 and 20\,m thresholds. 
 $\Delta$MRR: increase in MMR after re-ranking in 5\,m threshold.  }
\label{tab:place_recog_hard}
\end{center}
% \vspace{-5mm}
\end{table*}

==> chapters/tables/table_placog_original.tex <==
\begin{table*}[htb!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}}
%\hline
&  \multicolumn{4}{c}{MulRan Sejong} & \multicolumn{4}{c}{Apollo-SouthBay} & \multicolumn{4}{c}{KITTI}  \\
&  \multicolumn{2}{c}{5\,m thresh.} & \multicolumn{2}{c}{20\,m thresh.} 
&  \multicolumn{2}{c}{5\,m thresh.} & \multicolumn{2}{c}{20\,m thresh.} 
&  \multicolumn{2}{c}{5\,m thresh.} & \multicolumn{2}{c}{20\,m thresh.} 

\\
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}R@5\end{tabular}

\\[2pt]
\hline
MinkLoc3D*~\cite{Komorowski_2021_WACV} & 0.823 & 0.944 & 0.921 & 0.966 & 0.772 & 0.938 & 0.950 & 0.983 & 0.957 & 0.969 & 0.977 & 0.980  \\
DiSCO*~\cite{xu2021disco} & 0.940 & 0.975 & 0.958 & 0.981 & 
0.951 & 0.966 & 0.954 & 0.970 & 0.907 & 0.913 & 0.923 & 0.945  \\
DH3D*~\cite{du2020dh3d} & 0.324 & 0.562 & 0.589 & 0.755 & 0.253 & 0.496 & 0.504 & 0.707 &  0.755 & 0.911 & 0.868 & 0.961  \\
ScanContext~\cite{kim2018scan}  & 0.861 & 0.896 & 0.885 & 0.915 & 0.910 & 0.910 & 0.921 & 0.924 & 0.963 & 0.974 & 0.963 &  0.976 \\ 
Locus~\cite{vidanapathirana2020locus} & 	0.670 & 0.758 & 0.706 & 0.746 &  0.855 & 0.955 & 0.949 & 0.981 & 0.990 & 0.997 & 0.998 & \textbf{1.0}   \\
EgoNN~\cite{egonn} & 0.983 &  \textbf{0.999} &  \textbf{0.996} &  0.999 & 
0.957 & 0.977 & 0.963 & 0.982 & 
0.974 &  0.982 &  0.979 &  0.987
 \\

LCDNet~\cite{cattaneo2022lcdnet} &  0.631 & 0.820 & 0.858 & 0.921 & 0.647 & 0.817 & 0.874 & 0.921  &  0.969 & 0.994 & 0.995 & 0.998   \\
LoGG3D-Net~\cite{vid2022logg3d} & 0.977 & 0.997 & 0.988 & 0.998 &  0.952 & 0.984 & 0.982 & \underline{0.992} &  \textbf{0.997} & \textbf{0.998} & \textbf{1.0} & \textbf{1.0}   \\
\hline
EgoNN + SGV & \textbf{0.991} &  \textbf{0.999} &  \textbf{0.996} &  \textbf{1.0} & 
\underline{0.983} & \underline{0.987} & \underline{0.991} & \underline{0.992} & 
0.992 &  0.994 &  0.997 &  0.997
 \\
LCDNet + SGV & 0.908 & 0.924 & 0.943 & 0.958 &  0.900 & 0.908 & 0.952 & 0.956 &  \textbf{0.997} & 0.997 & \textbf{1.0} & \textbf{1.0}   \\
LoGG3D-Net + SGV & \underline{0.990} & \textbf{0.999} & 0.995 & \textbf{1.0} &  \textbf{0.986} & \textbf{0.993} & \textbf{0.996} & \textbf{0.996} &  \textbf{0.997} & \textbf{0.998} & \textbf{1.0} & \textbf{1.0} \\[2pt]
\end{tabular}
\caption{Place recognition on the `easy' evaluation set. 
% Recall@1 and Recall@5 are reported with 5 and 20\,m thresholds. 
(*) Results are obtained from \cite{egonn}.
Bold and underline represent the best and 2nd best result respectively in each column.}
\label{tab:place_recog_easy}
\end{center}
\end{table*}

==> chapters/tables/table_rerank_ablation.tex <==
\begin{table}[H]
  \centering
\begin{tabular}{l|cccc}

   & MulRan & Apollo & Kitii & Pittsburg  \\
	\hline 
    %  M2DP~\cite{He2016} & 00 & 00 & 00 \\
	 Normal & 0 & 0 & 0 & 0 \\
	 \hline
	 Global + average-QE~\cite{chum2007total} & 0 & 0 & 0 & 0 \\
	 Global + alpha-QE~\cite{radenovic2018cnnretrieval} & 0 & 0 & 0 & 0 \\
	 Global + k-reciprocal~\cite{qin2011hello,zhong2017re} & 0 & 0 & 0 & 0 \\
	 Global + region-diffusion~\cite{iscen2017efficient} & 0 & 0 & 0 & 0 \\
	 \hline
	 Local + RANSAC~\cite{fischler1981ransac} & 0 & 0 & 0 & 0 \\
	 Local + FGR~\cite{zhou2016fgr} & 0 & 0 & 0 & 0 \\
	 Local + Teaser~\cite{yang2020teaser} & 0 & 0 & 0 & 0 \\
	 \hline
	 Local + SM~\cite{spectralmatch} & 0 & 0 & 0 & 0 \\
	 Local + SC~\cite{bai2021pointdsc} & 0 & 0 & 0 & 0 \\
	 Local + SC2~\cite{chen2022sc2pcr} & 0 & 0 & 0 & 0 \\
% 	 MinkLoc3D~\cite{Kim2018} & 00 & 00 & 00 \\
	 \textbf{No-name (Ours)} & 0 & 0 & 0 & 0 \\
	\hline
\end{tabular}
\caption{Place recognition results under different re-ranking methods in the 4 datasets. Results reported are Recall@1. Rows are grouped as (1) global descriptor based re-ranking, (2) Robust estimators using local features, and (3) Spectral correspondence filtering with local features.
  }
  \label{tab:rerank_ablation}
\end{table}



==> chapters/tables/table_rerank_egonn.tex <==
% \begin{sidewaystable}
\begin{table*}[ht!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}|c@{\quad}c@{\quad}c@{\quad}c@{\quad}c}
%\hline
& &  \multicolumn{5}{c}{MulRan DCC}  & \multicolumn{5}{c}{ALITA}  & \multicolumn{5}{c}{KITTI-360} \\
& &  \multicolumn{2}{c}{5m} &  \multicolumn{2}{c}{20m} &  \multicolumn{1}{c}{}  &  \multicolumn{2}{c}{5m} &  \multicolumn{2}{c}{20m} &  \multicolumn{1}{c}{}  &  \multicolumn{2}{c}{5m} &  \multicolumn{2}{c}{20m} &  \multicolumn{1}{c}{} \\
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% \\
& \begin{tabular}{@{}c@{}}$n_{topk}$\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}t\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}t\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}t\end{tabular}

% Ew. dodać liczbę iteracji RANSACa jak w DH3D
\\[2pt]
\hline
% \Tstrut
Baseline  & - & 67.1 & 77.2 & 90.2 & 92.3 &  - & 79.8 & 87.3 & 91.7 &  94.9 & - & 86.9 & 90.1 &  88.2 & 91.4 & -  \\
\hline
\textit{(a) Global only:} &  &  &  &  &  &   &  &  &  &   &  &  &  &   &  & \\
Average-QE  & 2 & 67.4 & 76.7 & 90.2 & 91.8 &  0.2 & 79.8 & 86.5 & 91.7 &  94.3 & 0.1 & 86.9 & 89.3 &  88.2 & 90.8 & 0.2  \\
 & 20 & 35.2 & 47.6 & 54.7 & 65.0 &  0.2 & 13.1 & 27.4 & 26.2 &  44.0 & 0.1 & 46.2 & 59.4 &  49.7 & 63.8 & 0.2  \\
Alpha-QE \cite{radenovic2018cnnretrieval} & 2 & 67.4 & 76.7 & 90.6 & 92.0 &  0.2 & 81.0 & 87.1 & 92.9 &  94.9 & 0.1 & 86.7 & 89.2 &  87.9 & 90.6 & 0.2 \\
 & 20 & 34.5 & 47.4 & 54.7 & 65.0 &  0.3 & 13.1 & 28.4 & 26.2 &  45.0 & 0.2 & 47.0 & 59.9 &  50.8 & 64.4 & 0.3  \\
\hline
\textit{(b) GV: RIR}  &  &  &  &  &  &   &  &  &  &   &  &  &  &   &  & \\
RANSAC \cite{fischler1981ransac} & 2 & 71.0& 79.0 & 92.8 &  93.6 & 2.8 & 90.5 & 92.7 &  95.2 & 96.7 & 4.1 & 90.5 & 91.9 & 92.5 & 93.5  & 2.8 \\
 & 20 & \underline{72.0} & \underline{80.9} & \textbf{95.8} & \textbf{96.0} &  63.6 & \textbf{100} & \textbf{100} & \textbf{100} &  \textbf{100} & 60.4 & \underline{95.0} & \underline{96.4} &  \underline{98.5} & \underline{98.6} & 56.3  \\
FGR \cite{zhou2016fgr} & 2 & 70.4 & 78.7 & 91.2 & 92.8 &  79.7 & 89.3 & 92.1 & 95.2 &  96.7 & 54.8 & 90.2 & 91.7 &  92.2 & 93.4 & 74.4  \\
 & 20 & 70.7 & 78.9 & 92.2 & 93.2 &  175.7 & 97.6 & 98.8 & \textbf{100} &  \textbf{100} & 126.7 & 93.7 & 95.8 &  98.0 & 98.3 & 171.3  \\
TEASER++ \cite{yang2020teaser} & 2 & 70.0 & 78.5 & 92.5 & 93.4 &  26.3 & 90.5 & 92.7 & 95.2 &  96.7 & 30.1 & 89.9 & 91.6 &  92.2 & 93.4 & 35.1  \\
 & 20 & 71.3 & 80.6 & 93.8 & 94.8 &  261.3 & 98.8 & 99.4 & \textbf{100} &  \textbf{100} & 272.8 & 94.0 & 95.8 &  96.7 & 97.6 & 320.5  \\
\hline
\textit{(c) GV: SC}  &  &  &  &  &  &   &  &  &  &   &  &  &  &   &  & \\
\textbf{SpectralGV (Ours)} & 2 & 71.7 & 79.3 & 92.8 & 93.6 &  2.7 & 90.5 & 92.7 & 95.2 &  96.7 & 5.3 & 90.7 & 92.0  &  92.5 & 93.5 & 2.4  \\
 & 20 & \textbf{73.6} & \textbf{82.2} & \underline{95.1} & \underline{95.7} &  3.0 & \textbf{100} & \textbf{100} & \textbf{100} &  \textbf{100} & 5.7 & \textbf{95.7} & \textbf{96.9} &  \textbf{	98.7} & \textbf{98.8} & 2.8  \\[2pt]
\end{tabular}
\caption{
% \textcolor{red}{not about place recognition. re-ranking ablation .....have on the same page as fig. 3. focus discussion on this table}Place recognition results under different re-ranking methods using the EgoNN architecture. 
\textcolor{blue}{Comparison of re-ranking methods. The first row shows the baseline retrieval results without re-ranking.}
Methods in subsection (a) perform re-ranking using only the global descriptors. Methods in subsections (b) and (c) perform Geometric Verification (GV) based re-ranking where (b) computes the Registered-Inlier-Ratio (RIR) and (c) directly computes a Spatial Consistency (SC) score.
 %`R@1': Recall@1,  `MRR': Mean Reciprocal Rank, `t': time taken for re-ranking in ms, 
 $n_{topk}$: number of top-k retrieval candidates used during re-ranking.  %Time columns are not highlighted as time taken at different $n_{topk}$ values are incomparable. 
% Rows are grouped as (1) global descriptor based re-ranking, (2) Robust estimators using local features, and (3) Spectral correspondence filtering with local features.
}
\label{tab:rerank_egonn}
\end{center}
\end{table*}
% \end{sidewaystable}

==> chapters/tables/table_rerank_full.tex <==
% \begin{sidewaystable}
\begin{table*}[htb!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c}
%\hline
& \multicolumn{8}{c|}{EgoNN} & \multicolumn{8}{c}{LoGG3D-Net}  \\
&  \multicolumn{2}{c}{MulRan} & \multicolumn{2}{c}{Apollo} & \multicolumn{2}{c}{Kitti} & \multicolumn{2}{c|}{ALITA} &  \multicolumn{2}{c}{MulRan} & \multicolumn{2}{c}{Apollo} & \multicolumn{2}{c}{Kitti} & \multicolumn{2}{c}{ALITA} \\
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% \\
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
% Ew. dodać liczbę iteracji RANSACa jak w DH3D
\\[2pt]
\hline
% \Tstrut
Normal & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Global + average-QE~\cite{chum2007total} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + alpha-QE~\cite{radenovic2018cnnretrieval}  & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + k-reciprocal~\cite{qin2011hello,zhong2017re} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + region-diffusion~\cite{iscen2017efficient} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Local + RANSAC~\cite{fischler1981ransac} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Local + FGR~\cite{zhou2016fgr} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Local + Teaser~\cite{yang2020teaser} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Local + SM~\cite{spectralmatch} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
Local + SC~\cite{bai2021pointdsc} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
Local + SC2~\cite{chen2022sc2pcr} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
\textbf{No-name (Ours)} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\[2pt]
\end{tabular}
\caption{Place recognition results under different re-ranking methods in the 4 datasets. Results reported are Recall@1. Rows are grouped as (1) global descriptor based re-ranking, (2) Robust estimators using local features, and (3) Spectral correspondence filtering with local features.}
\label{tab:rerank_full}
\end{center}
\end{table*}
% \end{sidewaystable}

==> chapters/tables/table_rerank_full_sideways.tex <==
\begin{sidewaystable}
% \begin{table*}[htb!]

\begin{center}
\begin{tabular}{l@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c@{\quad}|c@{\quad}c}
%\hline
& \multicolumn{8}{c|}{EgoNN} & \multicolumn{8}{c}{LoGG3D-Net}  \\
&  \multicolumn{2}{c}{MulRan} & \multicolumn{2}{c}{Apollo} & \multicolumn{2}{c}{Kitti} & \multicolumn{2}{c|}{ALITA} &  \multicolumn{2}{c}{MulRan} & \multicolumn{2}{c}{Apollo} & \multicolumn{2}{c}{Kitti} & \multicolumn{2}{c}{ALITA} \\
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% &  \multicolumn{2}{c}{EgoNN} & \multicolumn{2}{c}{LoGG3D-Net} 
% \\
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
& \begin{tabular}{@{}c@{}}R@1\end{tabular}
& \begin{tabular}{@{}c@{}}MRR\end{tabular}
% Ew. dodać liczbę iteracji RANSACa jak w DH3D
\\[2pt]
\hline
% \Tstrut
Normal & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Global + average-QE~\cite{chum2007total} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + alpha-QE~\cite{radenovic2018cnnretrieval}  & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + k-reciprocal~\cite{qin2011hello,zhong2017re} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Global + region-diffusion~\cite{iscen2017efficient} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Local + RANSAC~\cite{fischler1981ransac} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Local + FGR~\cite{zhou2016fgr} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
Local + Teaser~\cite{yang2020teaser} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 & 0.0 & 0.0  \\
\hline

Local + SM~\cite{spectralmatch} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
Local + SC~\cite{bai2021pointdsc} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
Local + SC2~\cite{chen2022sc2pcr} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\
\textbf{No-name (Ours)} & 0.0 & 0.0 & 0.0 & 0.0 &  0 & 0 & 0 & 0 &  0.0 & 0.0 & 0.0 & 0.0  &  0.0 & 0.0 & 0.0 & 0.0 \\[2pt]
\end{tabular}
\caption{Place recognition results under different re-ranking methods in the 4 datasets. Results reported are Recall@1. Rows are grouped as (1) global descriptor based re-ranking, (2) Robust estimators using local features, and (3) Spectral correspondence filtering with local features.}
\label{tab:rerank_full}
\end{center}
% \end{table*}
\end{sidewaystable}

==> tables/Experiment1.tex <==

\begin{table*}[btp]
\centering
\begin{tabular}{l|clllllllllllll|}
\cline{2-15}
 &
  \multicolumn{14}{c|}{\ExperimentOne} \\ \cline{2-15} 
 &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \cline{2-15} 
 &
  CD                     & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
  \multicolumn{1}{l}{ 3.025} & \multicolumn{1}{l|}{0.0573} &
                      2.865 & \multicolumn{1}{l|}{0.100} &
                      5.617 & \multicolumn{1}{l|}{0.0727} &
                      0.602 & \multicolumn{1}{l|}{0.00780} &
                      4.622 & \multicolumn{1}{l|}{0.102} &
                      0.771 & \multicolumn{1}{l|}{0.0175} &
                      3.671 & 0.0438
   \\ \hline
   
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%   \multicolumn{1}{l}{0.9750} & \multicolumn{1}{l|}{0.0222} &
%                       2.145  & \multicolumn{1}{l|}{0.0750} &
%                       1.073  & \multicolumn{1}{l|}{0.0137} &
%                       0.4147 & \multicolumn{1}{l|}{0.00527} &
%                       0.7774 & \multicolumn{1}{l|}{0.0171} &
%                       0.4836 & \multicolumn{1}{l|}{0.0114} &
%                       0.9547 & 0.0114
%    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
  \multicolumn{1}{l}{0.212} & \multicolumn{1}{l|}{ 0.00437 } &
                     0.305  & \multicolumn{1}{l|}{ 0.0107  } &
                     0.192  & \multicolumn{1}{l|}{ 0.00249 } &
                     0.159  & \multicolumn{1}{l|}{ 0.00206 } &
                     0.182  & \multicolumn{1}{l|}{ 0.00401 } &
                     0.171  & \multicolumn{1}{l|}{ 0.00387 } &
                     0.263  &                      0.00314
   \\ \hline
\end{tabular}
\caption{  }
\label{tab:table1}
\end{table*}


==> tables/Experiment2.tex <==

\begin{table*}[btp]
\centering
\begin{tabular}{l|clllllllllllll|}
\cline{2-15}
 &
  \multicolumn{14}{c|}{\ExperimentTwo} \\ \cline{2-15} 
 &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \cline{2-15} &
  CD & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } & 
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } & 
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } & 
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
  \multicolumn{1}{l}{ 207.4 } & \multicolumn{1}{l|}{ 4.078 } &
                      229.7   & \multicolumn{1}{l|}{ 8.030 } &
                      218.3   & \multicolumn{1}{l|}{ 2.825 } &
                      183.2   & \multicolumn{1}{l|}{ 2.371 } &
                      205.1   & \multicolumn{1}{l|}{ 4.529 } &
                      171.6   & \multicolumn{1}{l|}{ 3.889 } &
                      236.3   &                      2.821   \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%   \multicolumn{1}{l}{ 0.8697 } & \multicolumn{1}{l|}{ 0.0215  } &
%                       2.353    & \multicolumn{1}{l|}{ 0.0823  } &
%                       0.3897   & \multicolumn{1}{l|}{ 0.00504 } &
%                       0.4363   & \multicolumn{1}{l|}{ 0.00565 } &
%                       0.7259   & \multicolumn{1}{l|}{ 0.0160  } &
%                       0.4198   & \multicolumn{1}{l|}{ 0.00951 } &
%                       0.8932   & 0.0107 \\ \hline

 \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
  \multicolumn{1}{l}{0.459} & \multicolumn{1}{l|}{0.0143} &
                     0.109  & \multicolumn{1}{l|}{0.0388} &
                     0.895  & \multicolumn{1}{l|}{0.0116} &
                     0.399  & \multicolumn{1}{l|}{0.00516} &
                     0.758  & \multicolumn{1}{l|}{0.0167} &
                     0.345  & \multicolumn{1}{l|}{0.00782} &
                     0.458  & 0.00547
   \\ \hline
\end{tabular}
\caption{  }
\label{tab:table2}
\end{table*}

==> tables/Experiment3.tex <==
\begin{table*}[btp]
\centering
\label{tab:my-table}
\begin{tabular}{l|clllllllllllll|}
\cline{2-15}
 &
  \multicolumn{14}{c|}{\ExperimentThree} \\ \cline{2-15} 
 &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \cline{2-15} 
 &
  CD &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
  \multicolumn{1}{l}{?} & \multicolumn{1}{l|}{?} &
                  ? & \multicolumn{1}{l|}{?} &
                  ? & \multicolumn{1}{l|}{?} &
                  ? & \multicolumn{1}{l|}{?} &
                  ? & \multicolumn{1}{l|}{?} &
                  ? & \multicolumn{1}{l|}{?} &
                  ? & ? \\ \hline

% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%   \multicolumn{1}{l}{ ? } & \multicolumn{1}{l|}{?} &
%                       ?   & \multicolumn{1}{l|}{?} &
%                       ?   & \multicolumn{1}{l|}{?} &
%                       ?   & \multicolumn{1}{l|}{?} &
%                       ?   & \multicolumn{1}{l|}{?} &
%                       ?   & \multicolumn{1}{l|}{?} &
%                       ?   &                     ? \\ \hline

\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
  \multicolumn{1}{l}{0.872} & \multicolumn{1}{l|}{0.0182} &
                     1.217  & \multicolumn{1}{l|}{0.0426} &
                     1.077  & \multicolumn{1}{l|}{0.0139} &
                     0.411  & \multicolumn{1}{l|}{0.00532} &
                     1.138  & \multicolumn{1}{l|}{0.0251} &
                     0.529  & \multicolumn{1}{l|}{0.0120} &
                     0.860  & 0.0103
   \\ \hline
\end{tabular}
\caption{  }
\end{table*}

==> tables/Experiment4.tex <==
\begin{table*}[btp]
\centering
\label{tab:my-table}
\begin{tabular}{|lllllllllllllll|}
\hline
\multicolumn{15}{|c|}{\ExperimentFour} \\ \hline
% \multicolumn{1}{|r|}{Shape} &
\multicolumn{1}{|r|}{ } &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \hline 
\multicolumn{1}{|l|}{ Method } &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} &
  \multicolumn{1}{c}{$\text{CD}$} & \multicolumn{1}{c|}{$\text{CD}_{m^2}$} \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
                  3.149  & \multicolumn{1}{l|}{0.0869} &
                  2.2863 & \multicolumn{1}{l|}{0.0327} &
                  0.6575 & \multicolumn{1}{l|}{0.0254} &
                  0.4485 & \multicolumn{1}{l|}{0.0173} &
                  0.8359 & \multicolumn{1}{l|}{0.0189} &
                  0.5123 & \multicolumn{1}{l|}{0.0113} &
                  1.0894 & \multicolumn{1}{l|}{0.0456} \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%                   0.794 & \multicolumn{1}{l|}{0.1160} &
%                   2.095 & \multicolumn{1}{l|}{0.0732} &
%                   0.395 & \multicolumn{1}{l|}{0.0051} &
%                   0.327 & \multicolumn{1}{l|}{0.0042} &
%                   0.585 & \multicolumn{1}{l|}{0.0129} &
%                   0.393 & \multicolumn{1}{l|}{0.0089} &
%                   0.969 & 0.0116 \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
                  0.579 & \multicolumn{1}{l|}{0.0138} &
                  1.286 & \multicolumn{1}{l|}{0.0449} &
                  0.296 & \multicolumn{1}{l|}{0.00383} &
                  0.261 & \multicolumn{1}{l|}{0.00337} &
                  0.770 & \multicolumn{1}{l|}{0.0170} &
                  0.304 & \multicolumn{1}{l|}{0.00690} &
                  0.559 & 0.00667 \\ \hline
\end{tabular}
\caption{ }
\end{table*}



==> tables/Experiment5.tex <==
\begin{table*}[btp]
\centering
\begin{tabular}{l|clllllllllllll|}
\cline{2-15} &
  \multicolumn{14}{c|}{\ExperimentFive} \\ \cline{2-15} &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \cline{2-15} &
  CD & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } & 
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} & \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } \\ \hline
  
\multicolumn{1}{|l|}{VIRDO} &
  % \multicolumn{1}{l}{3.868} & \multicolumn{1}{l|}{0.1114} &
  %                    8.219  & \multicolumn{1}{l|}{0.1176} &
  %                    6.321  & \multicolumn{1}{l|}{0.2442} &
  %                    0.8327 & \multicolumn{1}{l|}{0.03220} &
  %                    1.808  & \multicolumn{1}{l|}{0.04090} &
  %                    0.9436 & \multicolumn{1}{l|}{0.02080} &
  %                    5.085  & 0.2130 \\ \hline
  \multicolumn{1}{l}{375.8} & \multicolumn{1}{l|}{7.217} &
                     377.2  & \multicolumn{1}{l|}{13.19} &
                     322.4  & \multicolumn{1}{l|}{4.172} &
                     342.0  & \multicolumn{1}{l|}{4.427} &
                     341.0  & \multicolumn{1}{l|}{7.530} &
                     333.1  & \multicolumn{1}{l|}{7.548} &
                     539.1  & 6.436 \\ \hline
                     
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%   \multicolumn{1}{l}{ 249.1 } & \multicolumn{1}{l|}{  } &
%                       847.1   & \multicolumn{1}{l|}{  } &
%                        48.76  & \multicolumn{1}{l|}{  } &
%                         5.013 & \multicolumn{1}{l|}{  } &
%                         0.879 & \multicolumn{1}{l|}{  } &
%                       377.8   & \multicolumn{1}{l|}{  } &
%                       214.8   &                         \\ \hline
                       
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
    % \multicolumn{1}{l}{0.451} & \multicolumn{1}{l|}{0.00933} &
    %                    0.478  & \multicolumn{1}{l|}{0.0167} &
    %                    0.349  & \multicolumn{1}{l|}{0.00452} &
    %                    0.282  & \multicolumn{1}{l|}{0.00365} &
    %                    0.896  & \multicolumn{1}{l|}{0.0198} &
    %                    0.274  & \multicolumn{1}{l|}{0.00626} &
    %                    0.492  & 0.00512
    \multicolumn{1}{l}{1.993} & \multicolumn{1}{l|}{0.0442} &
                       2.906  & \multicolumn{1}{l|}{0.0102} &
                       2.046  & \multicolumn{1}{l|}{0.0265} &
                       0.954  & \multicolumn{1}{l|}{0.0123} &
                       3.906  & \multicolumn{1}{l|}{0.0863} &
                       1.205  & \multicolumn{1}{l|}{0.0273} &
                       0.944  & 0.0113
   \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}

==> tables/Experiment6.tex <==
\begin{table*}[btp]
\centering
\begin{tabular}{l|clllllllllllll|}
\cline{2-15}
 &
  \multicolumn{14}{c|}{\ExperimentSix} \\ \cline{2-15} 
 &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \cline{2-15} 
 &
  CD &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{ $\text{CD}_{m^{2}}$ } \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
  \multicolumn{1}{l}{ 362.7 } & \multicolumn{1}{l|}{  6.933 } &
                      359.5   & \multicolumn{1}{l|}{ 12.57  } &
                      305.1   & \multicolumn{1}{l|}{  3.949 } &
                      347.0   & \multicolumn{1}{l|}{  4.491 } &
                      314.1   & \multicolumn{1}{l|}{  6.938 } &
                      326.0   & \multicolumn{1}{l|}{  7.386 } &
                      521.0   &                       6.220   \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
%   \multicolumn{1}{l}{ 223.2 } & \multicolumn{1}{l|}{ 4.141 } &
%                       147.5   & \multicolumn{1}{l|}{ 5.156 } &
%                       457.1   & \multicolumn{1}{l|}{ 5.916 } &
%                       213.9   & \multicolumn{1}{l|}{ 2.769 } &
%                       273.3   & \multicolumn{1}{l|}{ 6.035 } &
%                       189.7   & \multicolumn{1}{l|}{ 4.299 } &
%                        78.15  &                      0.933   \\ \hline

\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Ours \end{tabular}} &
\multicolumn{1}{l}{5.80} & \multicolumn{1}{l|}{ 0.111  } &
                   6.24  & \multicolumn{1}{l|}{ 0.218  } &
                   9.56  & \multicolumn{1}{l|}{ 0.124  } &
                   2.71  & \multicolumn{1}{l|}{ 0.0354 } &
                   7.23  & \multicolumn{1}{l|}{ 0.160  } &
                   1.88  & \multicolumn{1}{l|}{ 0.0427 } &
                   7.75  &                      0.0925  \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}

==> tables/Experiment7.tex <==
\begin{table*}[btp]

\centering
\begin{tabular}{l|ll|}
\cline{2-3}
\multicolumn{1}{c|}{}                  & \multicolumn{2}{c|}{\ExperimentSeven} \\ \cline{2-3} 
\multicolumn{1}{r|}{}                  & \multicolumn{2}{c|}{Average}         \\ \cline{2-3} 
                                       & CD               & CDm2              \\ \hline
\multicolumn{1}{|l|}{VIRDO}            & ?                & ?                 \\ \hline

\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} &
? & ? \\ \hline
\multicolumn{1}{|l|}{Method II (ours)} & ?                & ?                 \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}

\end{table*}

==> tables/Experiment8.tex <==
\begin{table*}[btp]

\centering
\begin{tabular}{l|ll|}
\cline{2-3}
\multicolumn{1}{c|}{}                  & \multicolumn{2}{c|}{\ExperimentEight} \\ \cline{2-3} 
\multicolumn{1}{r|}{}                  & \multicolumn{2}{c|}{Average}         \\ \cline{2-3} 
                                       & CD               & CDm2              \\ \hline
\multicolumn{1}{|l|}{VIRDO}            & ?                & ?                 \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} Method I (ours)\end{tabular}} & ? & ? \\ \hline
\multicolumn{1}{|l|}{Method II (ours)} & 5.883                & 0.0761                 \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}

\end{table*}

==> tables/ExperimentResults_CD.tex <==
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{|l|llll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}}                         & \multicolumn{4}{c|}{Force withheld experiment, Metric: CD}                                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                & \multicolumn{1}{l|}{Random} & \multicolumn{1}{l|}{Lowest} & \multicolumn{1}{l|}{Highest} & Single Direction \\ \hline
VIRDO                                                                 & \multicolumn{1}{l|}{30.83}  & \multicolumn{1}{l|}{50.34}  & \multicolumn{1}{l|}{80.32}   & 60.48            \\ \hline
\begin{tabular}[c]{@{}l@{}}Shape-Space\\ Deformer (ours)\end{tabular} & \multicolumn{1}{l|}{1.031}  & \multicolumn{1}{l|}{0.862}  & \multicolumn{1}{l|}{1.831}   & 1.768            \\ \hline
\end{tabular}
\end{table}

==> tables/ExperimentResults_CD_and_CDm2.tex <==

\begin{table*}[btp]
\centering
\caption{}
\label{tab:exp_results}
\begin{tabular}{|c|clllllll|}
\hline
\multirow{3}{*}{Method}         & \multicolumn{8}{c|}{Force withheld experiment}                                                                                                                                                                                          \\ \cline{2-9} 
                                & \multicolumn{2}{c|}{Random}                              & \multicolumn{2}{c|}{Lowest}                              & \multicolumn{2}{c|}{Highest}      & \multicolumn{2}{c|}{Single Direction}                  \\ \cline{2-9} 
                                                  & \multicolumn{1}{c|}{CD}    & \multicolumn{1}{c|}{CDm2}   & \multicolumn{1}{c|}{CD}    & \multicolumn{1}{c|}{CDm2}   & \multicolumn{1}{c|}{CD}    & \multicolumn{1}{c|}{CDm2}   & \multicolumn{1}{c|}{CD}    & \multicolumn{1}{c|}{CDm2} \\ \hline
\multicolumn{1}{|l|}{\quad \; VIRDO}                     & \multicolumn{1}{l|}{30.83} & \multicolumn{1}{l|}{0.3360} & \multicolumn{1}{l|}{50.34} & \multicolumn{1}{l|}{0.3836} & \multicolumn{1}{l|}{80.32} & \multicolumn{1}{l|}{0.6462} & \multicolumn{1}{l|}{60.48} & 0.7130                    \\ \hline
\multicolumn{1}{|l|}{ \quad \; Shape-Space Deformer (ours) \quad \; } 
    & \multicolumn{1}{l|}{1.031} & \multicolumn{1}{l|}{0.0492} & \multicolumn{1}{l|}{0.862} & \multicolumn{1}{l|}{0.0716} & \multicolumn{1}{l|}{1.831} & \multicolumn{1}{l|}{0.0502} & \multicolumn{1}{l|}{1.768} & 0.0478                    \\ \hline
\end{tabular}
% \end{table}
\end{table*}

==> tables/ExperimentResults_CDm2.tex <==

\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{|l|llll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}}                         & \multicolumn{4}{c|}{Force withheld experiment, Metric: CD}                                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                & \multicolumn{1}{l|}{Random} & \multicolumn{1}{l|}{Lowest} & \multicolumn{1}{l|}{Highest} & Single Direction \\ \hline
VIRDO                                                                 & \multicolumn{1}{l|}{30.83}  & \multicolumn{1}{l|}{50.34}  & \multicolumn{1}{l|}{80.32}   & 60.48            \\ \hline
\begin{tabular}[c]{@{}l@{}}Shape-Space\\ Deformer (ours)\end{tabular} & \multicolumn{1}{l|}{1.031}  & \multicolumn{1}{l|}{0.862}  & \multicolumn{1}{l|}{1.831}   & 1.768            \\ \hline
\end{tabular}
\end{table}

==> tables/Experiments.tex <==
% With standard deviation:
\begin{table*}[t!]
	\centering
	\setlength{\tabcolsep}{5.0pt}
    \begin{tabular}{l cccc cccccccc c }
        \toprule
        \multicolumn{1}{c}{ }                       &
        \multicolumn{4}{c}{Shape Reconstruction}    &
        \multicolumn{8}{c}{Force Generalisation}    &
        \multicolumn{1}{c}{Object Generalisation}
        \\
        \multicolumn{1}{c}{ }                           &
        \multicolumn{2}{c}{\thead{Nominal}}             &
        \multicolumn{2}{c}{\thead{Deformed}}            &
        \multicolumn{2}{c}{\thead{Random}}              &
        \multicolumn{2}{c}{\thead{Lowest}}              &
        \multicolumn{2}{c}{\thead{Highest}}             &
        \multicolumn{2}{c}{\thead{Direction}}           &
        \multicolumn{1}{c}{\thead{One-object-blindfold}}
        \\
        \multicolumn{1}{c}{ }           &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}       &
        \multicolumn{1}{c}{$\sigma$}    &
        \multicolumn{1}{c}{$\mu$}
        \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-13} \cmidrule(lr){14-14}
        %
        % Method
        VIRDO~\cite{Youngsun_2022_VIRDO} &
        % Mean  Std dev
        0.7505 & 0.5751\hphantom{0} &
        0.7640 & 0.5890 &
        300.5  & 111.8  &
        0.9717 & 0.6847 &
        375.8  & 82.10  &
        362.1  & 80.42  &
        F \\
        %
        % Method
        Ours &
        % Mean  Std dev
        \textbf{0.2035} & \textbf{0.05293} &
        \textbf{0.4940} & \textbf{0.2868}  &
        \textbf{0.8720} & \textbf{0.3353}  &
        \textbf{0.5793} & \textbf{0.3984}  &
        \textbf{1.993}  & \textbf{1.208}   &
        \textbf{5.895}  & \textbf{3.001}   &
        \textbf{5.883}
        \\
    	\bottomrule
	\end{tabular}
    %
	\caption{
        Our method (Ours) can produce better reconstructions, generalise to a wider range of applied forces, and is more robust to sample size than the next best method for predicting shape deformation (VIRDO~\cite{Youngsun_2022_VIRDO}).
        All metrics are mean L2 Chamfer Distance (CD $\downarrow$) between mesh reconstructions and ground truth point clouds.
        \textbf{CD results are multiplied by} $\mathbf{10^{3}}$ for readability, as in \cite{Youngsun_2022_VIRDO}, with both mean and standard deviation given.
        F indicates inability to produce a watertight reconstruction.
    }
	\label{tab:results}
\end{table*}


\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{5.0pt}
    \begin{tabular}{l cc}
        \toprule
        \multicolumn{1}{c}{ }                       &
        \multicolumn{2}{c}{Shape Reconstruction}    \\
        \multicolumn{1}{c}{ }                           &
        \thead{Nominal}             &
        \thead{Deformed}            \\
        \cmidrule(lr){2-3}
        %
        VIRDO~\cite{Youngsun_2022_VIRDO} &
        $0.7505 \pm 0.5751$ &
        $0.7640 \pm 0.5890$ \\
        %
        Ours &
        $\mathbf{0.2035} \pm \mathbf{0.05293}$ &
        $\mathbf{0.4940} \pm \mathbf{0.2868}$ \\
    	\bottomrule
	\end{tabular}
    %
	\caption{
        Shape reconstruction comparison between our method and VIRDO. 
        All metrics are mean L2 Chamfer Distance (CD $\downarrow$) between mesh reconstructions and ground truth point clouds.
        \textbf{CD results are multiplied by} $\mathbf{10^{3}}$ for readability.
    }
	\label{tab:shape-reconstruction}
\end{table}

\begin{table}[t!]
	\centering
	% \setlength{\tabcolsep}{1.5pt} % Keep reduced column padding
	\setlength{\tabcolsep}{2.0pt} % Keep reduced column padding
    \scriptsize % Further reduce font size
    \begin{tabular}{l cccc}
        \toprule
        \multicolumn{1}{c}{ }                       &
        \multicolumn{4}{c}{Force Generalisation}    \\
        \multicolumn{1}{c}{ }                           &
        \thead{Random}              &
        \thead{Lowest}              &
        \thead{Highest}             &
        \thead{Direction}           \\
        \cmidrule(lr){2-5}
        %
        VIRDO &
        $300.5 \pm 111.80$  &
        $0.972 \pm 0.69$ &
        $375.8 \pm 82.10$  &
        $362.1 \pm 80.42$  \\
        %
        Ours &
        $\mathbf{0.872} \pm \mathbf{0.34}$ &
        $\mathbf{0.579} \pm \mathbf{0.40}$ &
        $\mathbf{1.993} \pm \mathbf{1.21}$  &
        $\mathbf{5.895} \pm \mathbf{3.00}$  \\
    	\bottomrule
	\end{tabular}
    %
	\caption{
        Force generalisation comparison between our method and VIRDO.
        All metrics are mean L2 Chamfer Distance (CD $\downarrow$).
        \textbf{CD results are multiplied by} $\mathbf{10^{3}}$ for readability.
    }
	\label{tab:force-generalisation}
\end{table}


\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{5.0pt}
    \begin{tabular}{l c }
        \toprule

        VIRDO~\cite{Youngsun_2022_VIRDO} &
        F \\
        %
        Ours &
        $\mathbf{5.883}$ \\
    	\bottomrule
	\end{tabular}
    %
	\caption{
        Object generalisation comparison between our method and VIRDO.
        All metrics are mean L2 Chamfer Distance (CD $\downarrow$).
        \textbf{CD results are multiplied by} $\mathbf{10^{3}}$ for readability.
    }
	\label{tab:object-generalisation}
\end{table}


% \begin{table*}[t!]
% 	\centering
% 	% \resizebox{\textwidth}{!}{
% 	\setlength{\tabcolsep}{2pt}
% 	% \begin{tabular}{l cc cccc c ccccc}
%     \begin{tabular}{l cc cccc c }
%         \toprule
%         % & \multicolumn{2}{c}{Shape Reconstruction} & \multicolumn{4}{c}{Force Generalisation} & \multicolumn{1}{c}{Robustness to Sample Size}\\
%         & \multicolumn{2}{c}{Shape Reconstruction} & \multicolumn{4}{c}{Force Generalisation} & \multicolumn{1}{c}{Object Generalisation}\\

%         & \thead{Nominal} & \thead{Deformed}
%         & \thead{Random-\\forces-withheld} &\thead{Lowest-magnitude-\\forces-withheld} & \thead{Highest-magnitude-\\forces-withheld} & \thead{Single-direction-\\forces-withheld}
%         & \thead{ One-object-\\blindfold}  \\


%         \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-8}

%         VIRDO~\cite{Youngsun_2022_VIRDO}      & 0.750 & 0.764 & 30.83 & 3.149 & 375.8 & 362.7 & F \\
%         % Ours - SDF & 0.975 &        &  &  &  &  &  \\
%         Ours       & \textbf{0.212} & \textbf{0.459} & \textbf{0.872} & \textbf{0.579} & \textbf{1.993} & \textbf{5.80} & \textbf{5.883} \\
        
%     	\bottomrule
% 	\end{tabular}
% 	% }
% 	\caption{Our method (Ours) can produce better reconstructions, generalise to a wider range of applied forces, and is more robust to sample size than the next best method for predicting shape deformation (VIRDO\cite{Youngsun_2022_VIRDO}). All metrics are L2 Chamfer Distance (CD) between mesh reconstructions and ground truth point clouds. F indicates unable to produce a watertight reconstruction.}
% 	\label{tab:results}
% \end{table*}



==> tables/empty_table.tex <==
\begin{table*}[btp]

\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{|lllllllllllllll|}
\hline
\multicolumn{15}{|c|}{\ExperimentFour} \\ \hline
\multicolumn{1}{|r|}{Shape} &
  \multicolumn{2}{c|}{Average} &
  \multicolumn{2}{c|}{Shape 0} &
  \multicolumn{2}{c|}{Shape 1} &
  \multicolumn{2}{c|}{Shape 2} &
  \multicolumn{2}{c|}{Shape 3} &
  \multicolumn{2}{c|}{Shape 4} &
  \multicolumn{2}{c|}{Shape 5} \\ \hline 
\multicolumn{1}{|l|}{Method} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} &
  \multicolumn{1}{c}{CD} &
  \multicolumn{1}{c|}{CDm2} \\ \hline
\multicolumn{1}{|l|}{VIRDO} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  ? \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Shape-Space \\ Deformer (ours)\end{tabular}} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  \multicolumn{1}{l|}{?} &
  ? &
  ? \\ \hline
\end{tabular}

\end{table*}

==> tables/explicit_vs_implicit_fields.tex <==

\begin{table}
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{cllcl}
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{Field} &
  \multicolumn{1}{c}{Input} &
  Output &
  \multicolumn{1}{c}{Objective} \\ \cline{2-5} 
\multicolumn{1}{c|}{\multirow{2}{*}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ Implicit }}}} &
  \multicolumn{1}{l|}{SDF} &
  \multicolumn{1}{l|}{$\mathbf{x} \in \mathbb{R}^{3}$} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Signed \\ distance\\ $s \in \mathbb{R}$\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$\mathbf{x}_{i}$ such that\\ $\text{SDF}(\mathbf{x}_{i}) = 0$\end{tabular}} \\ \cline{2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{NeRF} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$\mathbf{x} \in \mathbb{R}^{3}$\\ $\mathbf{d} \in \mathbb{SE}(3)$\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Point density\\ $\sigma_{i} \in \mathbb{R}$\\ and colour\\ $\mathbf{c}_{i} \in \mathbb{R}^{3}$\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} Accumulated colour \\ $C \in \mathbb{R}^{3}$ rendered from \\ ${ \nerfRenderingEqn }$\end{tabular}} \\ \cline{2-5} 
\multicolumn{1}{c|}{\multirow{3}{*}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ Explicit }}}} &
  \multicolumn{1}{l|}{Image} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Pixel\\ $\mathbf{p} \in \mathbb{R}^{2}$\end{tabular}} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}RGB colour\\ $c \in \mathbb{R}^{3}$\end{tabular}} \\ \cline{2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{ENS} &
  \multicolumn{1}{l|}{$\mathbf{x} \in \mathbb{R}^{3}$} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Surface point\\ $\mathbf{x}' \in \mathbb{R}^{3}$\end{tabular}} \\ \cline{2-5} 
\multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{Deform} &
  \multicolumn{1}{l|}{$\mathbf{x} \in \mathbb{R}^{3}$} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Deformation vector\\ $\mathbf{d} \in \mathbb{R}^{3}$\end{tabular}} \\ \cline{2-5} 
\end{tabular}
\caption{ Explicit vs. Implicit \emph{Use} of Neural Fields}
\hl{This table is just an idea, don't shoot me for it!}
\label{tab:explicit_vs_implicit_fields}
\end{table}

==> tables/models_comparison.tex <==
% \begin{table*}[btp]
% \centering
% \begin{tabular}{|ll|rl|r|r|r|r|r|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{Method}} &
%   \multicolumn{2}{c|}{Data Samples} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Epochs}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Steps}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Parameters}} &
%   \multicolumn{1}{c|}{Training} &
%   \multicolumn{1}{c|}{Rendering} \\ \cline{3-4}
% \multicolumn{2}{|c|}{} &
%   Count &
%   \multicolumn{1}{c|}{Type} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{Time (Hr)} &
%   \multicolumn{1}{c|}{Time (s)} \\ \hline
% \multirow{3}{*}{VIRDO}  & Pre-training  & 6   & nominal  & 10,000 & 60,000  & 34.3M & 1.488 & $\sim$5.0 \\ \cline{2-2}
%                         & Main-training & 144 & deformed & 4,000  & 576,000 & 18.3M & 7.291 & 5.0 \\ \cline{2-2}
%                         & Total         &     &          &        & 636,000 & 52.6M & 8.779 & 5.0 \\ \hline
% % \multicolumn{2}{|l|}{SDF Method (ours)} & 150 & deformed & 2000   & 300,000 & 52.1M & 7.678 & $\sim$5.0 \\ \hline
% % \multicolumn{2}{|l|}{NVF Method (ours) 1} & 150 & deformed & 300    & 45,000  & 1.0M  & 0.450 & $\sim$0.2 \\ \hline
% % \multicolumn{2}{|l|}{NVF Method (ours) 2} & 150 & deformed & 300    & 45,000  & 317k  & 0.450 & $\sim$0.5 \\ \hline
% \multicolumn{2}{|l|}{Ours} & 150 & deformed & 300    & 45,000  & 1.0M  & 0.450 & 0.2 \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:model-efficiency}
% \end{table*}


\begin{table*}[t!]
\centering
\begin{tabular}{ll|r|r|r|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{Method}} &
  % \multicolumn{2}{c|}{Data Samples} &
  % \multicolumn{1}{c|}{\multirow{2}{*}{Epochs}} &
  % \multicolumn{1}{c|}{\multirow{2}{*}{Steps}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Parameters}} &
  \multicolumn{1}{c|}{Training} &
  \multicolumn{1}{c|}{Rendering} \\ 
  % \cline{3-4}
\multicolumn{2}{|c|}{} &
  % Count &
  % \multicolumn{1}{c|}{Type} &
  % \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  % \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{Time (Hr)} &
  \multicolumn{1}{c|}{Time (s)} \\ \hline
\multicolumn{2}{|l|}{VIRDO}   &   52.6M & 8.779 & 5.0 \\ %\hline
\multicolumn{2}{|l|}{Ours} & 1.0M  & 0.450 & 0.2 \\ \hline
\end{tabular}
\caption{Model parameter, training and inference times comparison.}
\label{tab:model-efficiency}
\end{table*}


